Formal Verification of Multi-Paxos for Distributed Consensus

Paxos is an important algorithm for a set of distributed processes to agree on a single value or a sequence of values, for which it is called Basic Paxos or Multi-Paxos, respectively. Consensus is critical when distributed services are replicated for fault-tolerance, because non-faulty replicas must agree on the state of the system or the sequence of operations that have been performed. Unfortunately, consensus algorithms including Multi-Paxos in particular are well-known to be difficult to understand, and their accurate specifications and correctness proofs remain challenging, despite extensive studies ever since Lamport introduced Paxos. This article describes formal specification and verification of Lamport's Multi-Paxos algorithm for distributed consensus. The specification is written in TLA+, Lamport's Temporal Logic of Actions. The proof is written and automatically checked using TLAPS, the TLA+ Proof System. The proof is for the safety property of the algorithm. Building on Lamport, Merz, and Doligez's specification and proof for Basic Paxos, we aim to facilitate the understanding of Multi-Paxos and its proof by minimizing the difference from those for Basic Paxos, and to demonstrate a general way of proving other variants of Paxos and other sophisticated distributed algorithms. We also discuss our general strategies and results for proving complex invariants using invariance lemmas and increments, for proving properties about sets and tuples to help the proof check succeed in significantly reduced time, and for overall proof improvement leading to considerably reduced proof size.

==> PaxosTLAPS_tla.tex <==
%%%\batchmode %% Suppresses most terminal output.
%%%\documentclass[format=acmsmall, review=false, screen=true]{acmart}
%%%\usepackage{amssymb}
%%%\usepackage{dsfont}
%%%\usepackage{xcolor}
%%%\usepackage[T1]{fontenc}
%%%\usepackage{letltxmacro}
%%%\usepackage{scalefnt}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.15}#1}}
\definecolor{boxshade}{gray}{0.85}
%%%\usepackage{latexsym}
%%%\usepackage{ifthen}
% \usepackage{color}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SWITCHES                                                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboolean{tlashading} 
\setboolean{tlashading}{true}
\makeatletter
 %% this is needed only when inserted into the file, not when
 %% used as a package file.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                           %
% DEFINITIONS OF SYMBOL-PRODUCING COMMANDS                                  %
%                                                                           %
%    TLA+      LaTeX                                                        %
%    symbol    command                                                      %
%    ------    -------                                                      %
%    =>        \implies                                                     %
%    <:        \ltcolon                                                     %
%    :>        \colongt                                                     %
%    ==        \defeq                                                       %
%    ..        \dotdot                                                      %
%    ::        \coloncolon                                                  %
%    =|        \eqdash                                                      %
%    ++        \pp                                                          %
%    --        \mm                                                          %
%    **        \stst                                                        %
%    //        \slsl                                                        %
%    ^         \ct                                                          %
%    \A        \A                                                           %
%    \E        \E                                                           %
%    \AA       \AA                                                          %
%    \EE       \EE                                                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\symlength}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\ltcolon}{\mathrel{<\!\!\mbox{\footnotesize:}}}
\newcommand{\colongt}{\mathrel{\!\mbox{\footnotesize:}\!\!>}}
\newcommand{\defeq}{\;\mathrel{\smash{\triangleq}}\,}
%\renewcommand{\defeq}{\;\mathrel{\smash   %% keep this symbol from being too tall
%   {{\stackrel{\scriptscriptstyle\Delta}{=}}}}\;}
\newcommand{\dotdot}{\mathrel{\ldotp\ldotp}}
\newcommand{\coloncolon}{\mathrel{::\;}}
\newcommand{\eqdash}{\mathrel = \joinrel \hspace{-.28em}|}
\newcommand{\pp}{\mathbin{++}}
\newcommand{\mm}{\mathbin{--}}
\newcommand{\stst}{*\!*}
\newcommand{\slsl}{/\!/}
\newcommand{\ct}{\hat{\hspace{.4em}}}
\renewcommand{\A}{\forall}
\renewcommand{\E}{\exists}
\renewcommand{\AA}{\makebox{$\raisebox{.05em}{\makebox[0pt][l]{%
   $\forall\hspace{-.517em}\forall\hspace{-.517em}\forall$}}%
   \forall\hspace{-.517em}\forall \hspace{-.517em}\forall\,$}}
\renewcommand{\EE}{\makebox{$\raisebox{.05em}{\makebox[0pt][l]{%
   $\exists\hspace{-.517em}\exists\hspace{-.517em}\exists$}}%
   \exists\hspace{-.517em}\exists\hspace{-.517em}\exists\,$}}
\newcommand{\whileop}{\.{\stackrel
  {\mbox{\footnotesize\raisebox{-.3em}[0pt][0pt]{$\scriptscriptstyle+\;\,$}}}%
  {-\hspace{-.16em}\triangleright}}}

% Commands are defined to produce the upper-case keywords.
% Note that some have space after them.
\renewcommand{\ASSUME}{\textcolor{purple}{{\textsc{assume }}}}
\renewcommand{\ASSUMPTION}{\textcolor{purple}{{\textsc{assumption }}}}
\renewcommand{\AXIOM}{\textcolor{purple}{{\textsc{axiom }}}}
\renewcommand{\BOOLEAN}{\textcolor{purple}{{\textsc{boolean }}}}
\renewcommand{\CASE}{\textcolor{purple}{{\textsc{ case }}}}
\renewcommand{\CONSTANT}{\textcolor{purple}{{\textsc{constant }}}}
\renewcommand{\CONSTANTS}{\textcolor{purple}{{\textsc{constants }}}}
\renewcommand{\ELSE}{\settowidth{\symlength}{\THEN}%
   \makebox[\symlength][l]{\textcolor{purple}{{\textsc{ else}}}}}
\renewcommand{\EXCEPT}{\textcolor{purple}{{\textsc{ except }}}}
\renewcommand{\EXTENDS}{\textcolor{purple}{{\textsc{extends }}}}
\renewcommand{\FALSE}{\textcolor{purple}{{\textsc{false}}}}
\renewcommand{\IF}{\textcolor{purple}{{\textsc{if }}}}
\renewcommand{\IN}{\settowidth{\symlength}{\LET}%
   \makebox[\symlength][l]{\textcolor{purple}{{\textsc{in}}}}}
\renewcommand{\INSTANCE}{\textcolor{purple}{{\textsc{instance }}}}
\renewcommand{\LET}{\textcolor{purple}{{\textsc{let }}}}
\renewcommand{\LOCAL}{\textcolor{purple}{{\textsc{local }}}}
\newcommand{\MODULE}{\textcolor{purple}{{\textsc{module }}}}
\renewcommand{\OTHER}{\textcolor{purple}{{\textsc{other }}}}
\renewcommand{\STRING}{\textcolor{purple}{{\textsc{string}}}}
\renewcommand{\THEN}{\textcolor{purple}{{\textsc{ then }}}}
\renewcommand{\THEOREM}{\textcolor{purple}{{\textsc{theorem }}}}
\renewcommand{\LEMMA}{\textcolor{purple}{{\textsc{lemma }}}}
\renewcommand{\PROPOSITION}{\textcolor{purple}{{\textsc{proposition }}}}
\newcommand{\COROLLARY}{\textcolor{purple}{{\textsc{corollary }}}}
\renewcommand{\TRUE}{\textcolor{purple}{{\textsc{true}}}}
\renewcommand{\VARIABLE}{\textcolor{purple}{{\textsc{variable }}}}
\renewcommand{\VARIABLES}{\textcolor{purple}{{\textsc{variables }}}}
\renewcommand{\WITH}{\textcolor{purple}{{\textsc{ with }}}}
\renewcommand{\WF}{\textrm{WF}}
\renewcommand{\SF}{\textrm{SF}}
\renewcommand{\CHOOSE}{\textcolor{purple}{{\textsc{choose }}}}
\renewcommand{\ENABLED}{\textcolor{purple}{{\textsc{enabled }}}}
\renewcommand{\UNCHANGED}{\textcolor{purple}{{\textsc{unchanged }}}}
\renewcommand{\SUBSET}{\textcolor{purple}{{\textsc{subset }}}}
\renewcommand{\UNION}{\textcolor{purple}{{\textsc{union }}}}
\renewcommand{\DOMAIN}{\textcolor{purple}{{\textsc{domain }}}}
% Added for tla2tex
\renewcommand{\BY}{\textcolor{purple}{{\textsc{by }}}}
\renewcommand{\OBVIOUS}{\textcolor{purple}{{\textsc{obvious }}}}
\renewcommand{\HAVE}{\textcolor{purple}{{\textsc{have }}}}
\renewcommand{\QED}{\textcolor{purple}{{\textsc{qed }}}}
\renewcommand{\TAKE}{\textcolor{purple}{{\textsc{take }}}}
\renewcommand{\DEF}{\textcolor{purple}{{\textsc{ def }}}}
\renewcommand{\HIDE}{\textcolor{purple}{{\textsc{hide }}}}
\renewcommand{\RECURSIVE}{\textcolor{purple}{{\textsc{recursive }}}}
\renewcommand{\USE}{\textcolor{purple}{{\textsc{use }}}}
\renewcommand{\DEFINE}{\textcolor{purple}{{\textsc{define }}}}
\renewcommand{\PROOF}{\textcolor{purple}{{\textsc{proof }}}}
\renewcommand{\WITNESS}{\textcolor{purple}{{\textsc{witness }}}}
\renewcommand{\PICK}{\textcolor{purple}{{\textsc{pick }}}}
\renewcommand{\DEFS}{\textcolor{purple}{{\textsc{defs }}}}
\renewcommand{\PROVE}{\settowidth{\symlength}{\ASSUME}%
   \makebox[\symlength][l]{\textcolor{purple}{{\textsc{prove}}\@s{-3.28}}}}
  %% The \@s{-4.1) is a kludge added on 24 Oct 2009 [happy birthday, Ellen]
  %% so the correct alignment occurs if the user types
  %%   ASSUME X
  %%   PROVE  Y
  %% because it cancels the extra 4.1 pts added because of the 
  %% extra space after the PROVE.  This seems to works OK.
  %% However, the 4.1 equals Parameters.LaTeXLeftSpace(1) and
  %% should be changed if that method ever changes.
\renewcommand{\SUFFICES}{\textcolor{purple}{{\textsc{suffices }}}}
\renewcommand{\NEW}{\textcolor{purple}{{\textsc{new }}}}
\renewcommand{\LAMBDA}{\textcolor{purple}{{\textsc{lambda }}}}
\renewcommand{\STATE}{\textcolor{purple}{{\textsc{state }}}}
\renewcommand{\ACTION}{\textcolor{purple}{{\textsc{action }}}}
\renewcommand{\TEMPORAL}{\textcolor{purple}{{\textsc{temporal }}}}
\newcommand{\ONLY}{\textcolor{purple}{{\textsc{only }}              }}
\renewcommand{\OMITTED}{\textcolor{purple}{{\textsc{omitted }}        }}
\newcommand{\@pfstepnum}[2]{\ensuremath{\langle#1\rangle}\textrm{#2}}
\newcommand{\bang}{\@s{0.8}\mbox{\footnotesize\small !}\@s{0.8}}
%% We should format || differently in PlusCal code than in TLA+ formulas.
\newcommand{\p@barbar}{\ifpcalsymbols
   \,\,\rule[-.25em]{.075em}{1em}\hspace*{.2em}\rule[-.25em]{.075em}{1em}\,\,%
   \else \,||\,\fi}
%% PlusCal keywords
\newcommand{\p@fair}{\textbf{fair }}
\newcommand{\p@semicolon}{\textbf{\,; }}
\newcommand{\p@algorithm}{\textbf{algorithm }}
\newcommand{\p@mmfair}{\textbf{-{}-fair }}
\newcommand{\p@mmalgorithm}{\textbf{-{}-algorithm }}
\newcommand{\p@assert}{\textbf{assert }}
\newcommand{\p@await}{\textbf{await }}
\newcommand{\p@begin}{\textbf{begin }}
\newcommand{\p@end}{\textbf{end }}
\newcommand{\p@call}{\textbf{call }}
\newcommand{\p@define}{\textbf{define }}
\newcommand{\p@do}{\textbf{ do }}
\newcommand{\p@either}{\textbf{either }}
\newcommand{\p@or}{\textbf{or }}
\newcommand{\p@goto}{\textbf{goto }}
\newcommand{\p@if}{\textbf{if }}
\newcommand{\p@then}{\,\,\textbf{then }}
\newcommand{\p@else}{\ifcsyntax \textbf{else } \else \,\,\textbf{else }\fi}
\newcommand{\p@elsif}{\,\,\textbf{elsif }}
\newcommand{\p@macro}{\textbf{macro }}
\newcommand{\p@print}{\textbf{print }}
\newcommand{\p@procedure}{\textbf{procedure }}
\newcommand{\p@process}{\textbf{process }}
\newcommand{\p@return}{\textbf{return}}
\newcommand{\p@skip}{\textbf{skip}}
\newcommand{\p@variable}{\textbf{variable }}
\newcommand{\p@variables}{\textbf{variables }}
\newcommand{\p@while}{\textbf{while }}
\newcommand{\p@when}{\textbf{when }}
\newcommand{\p@with}{\textbf{with }}
\newcommand{\p@lparen}{\textbf{(\,\,}}
\newcommand{\p@rparen}{\textbf{\,\,) }}   
\newcommand{\p@lbrace}{\textbf{\{\,\,}}   
\newcommand{\p@rbrace}{\textbf{\,\,\} }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% REDEFINE STANDARD COMMANDS TO MAKE THEM FORMAT BETTER %
%                                                       %
% We redefine \in and \notin                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\_}{\rule{.4em}{.06em}\hspace{.05em}}
\newlength{\equalswidth}
\let\oldin=\in
\let\oldnotin=\notin
\renewcommand{\in}{%
   {\settowidth{\equalswidth}{$\.{=}$}\makebox[\equalswidth][c]{$\oldin$}}}
\renewcommand{\notin}{%
   {\settowidth{\equalswidth}{$\.{=}$}\makebox[\equalswidth]{$\oldnotin$}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                  %
% HORIZONTAL BARS:                                 %
%                                                  %
%   \moduleLeftDash    |~~~~~~~~~~                 %
%   \moduleRightDash    ~~~~~~~~~~|                %
%   \midbar            |----------|                %
%   \bottombar         |__________|                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\charwidth}\settowidth{\charwidth}{{\small\tt M}}
\setlength{\boxrulewd}{.4pt}
\setlength{\boxlineht}{.5\baselineskip}
\renewcommand{\boxsep}{\charwidth}
\setlength{\boxruleht}{.5ex}
\setlength{\boxruledp}{-\boxruleht}
\addtolength{\boxruledp}{\boxrulewd}
\renewcommand{\boxrule}{\leaders\hrule height \boxruleht depth \boxruledp
                      \hfill\mbox{\footnotesize}}
\renewcommand{\@computerule}{%
  \setlength{\boxruleht}{.5ex}%
  \setlength{\boxruledp}{-\boxruleht}%
  \addtolength{\boxruledp}{\boxrulewd}}

\renewcommand{\bottombar}{\hspace{-\boxsep}%
  \raisebox{-\boxrulewd}[0pt][0pt]{\rule[.5ex]{\boxrulewd}{\boxlineht}}%
  \boxrule
  \raisebox{-\boxrulewd}[0pt][0pt]{%
      \rule[.5ex]{\boxrulewd}{\boxlineht}}\hspace{-\boxsep}\vspace{0pt}}

\newcommand{\moduleLeftDash}%
   {\hspace*{-\boxsep}%
     \raisebox{-\boxlineht}[0pt][0pt]{\rule[.5ex]{\boxrulewd
               }{\boxlineht}}%
    \boxrule\hspace*{.4em }}

\newcommand{\moduleRightDash}%
    {\hspace*{.4em}\boxrule
    \raisebox{-\boxlineht}[0pt][0pt]{\rule[.5ex]{\boxrulewd
               }{\boxlineht}}\hspace{-\boxsep}}%\vspace{.2em}

\renewcommand{\midbar}{\hspace{-\boxsep}\raisebox{-.5\boxlineht}[0pt][0pt]{%
   \rule[.5ex]{\boxrulewd}{\boxlineht}}\boxrule\raisebox{-.5\boxlineht%
   }[0pt][0pt]{\rule[.5ex]{\boxrulewd}{\boxlineht}}\hspace{-\boxsep}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FORMATING COMMANDS                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PLUSCAL tlashading                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The TeX pcaltlashading switch is set on to cause PlusCal tlashading to be
% performed.  This changes the behavior of the following commands and
% environments to cause full-width tlashading to be performed on all lines.
% 
%   \tstrut \@x cpar mcom \@pvspace
% 
% The TeX pcalsymbols switch is turned on when typesetting a PlusCal algorithm,
% whether or not tlashading is being performed.  It causes symbols (other than
% parentheses and braces and PlusCal-only keywords) that should be typeset
% differently depending on whether they are in an algorithm to be typeset
% appropriately.  Currently, the only such symbol is "||".
%
% The TeX csyntax switch is turned on when typesetting a PlusCal algorithm in
% c-syntax.  This allows symbols to be format differently in the two syntaxes.
% The "else" keyword is the only one that is.

\newif\ifpcaltlashading \pcaltlashadingfalse
\newif\ifpcalsymbols \pcalsymbolsfalse
\newif\ifcsyntax     \csyntaxtrue

% The \@pvspace command makes a vertical space.  It uses \vspace
% except with \ifpcaltlashading, in which case it sets \pvcalvspace
% and the space is added by a following \@x command.
%
\setlength{\pcalvspace}{0pt}%
\renewcommand{\@pvspace}[1]{%
  \ifpcaltlashading
     \par\global\setlength{\pcalvspace}{#1}%
  \else
     \par\vspace{#1}%
  \fi
}

% The lcom environment was changed to set \lcomindent equal to
% the indentation it produces.  This length is used by the
% cpar environment to make tlashading extend for the full width
% of the line.  This assumes that lcom environments are not
% nested.  I hope TLATeX does not nest them.
%
\setlength{\lcomindent}{0pt}%

%\tstrut: A strut to produce inter-paragraph space in a comment.
%\rstrut: A strut to extend the bottom of a one-line comment so
%         there's no break in the tlashading between comments on 
%         successive lines.
\renewcommand\tstrut%
  {\raisebox{\vshadelen}{\raisebox{-.25em}{\rule{0pt}{1.15em}}}%
   \global\setlength{\vshadelen}{0pt}}
\renewcommand\rstrut{\raisebox{-.25em}{\rule{0pt}{1.15em}}%
 \global\setlength{\vshadelen}{0pt}}


% \.{op} formats operator op in math mode with empty boxes on either side.
% Used because TeX otherwise vary the amount of space it leaves around op.
\renewcommand{\.}[1]{\ensuremath{\mbox{\footnotesize}#1\mbox{\footnotesize}}}

% \@s{n} produces an n-point space
\renewcommand{\@s}[1]{\hspace{#1pt}}           

% \@x{txt} starts a specification line in the beginning with txt
% in the final LaTeX source.
\renewcommand\xtstrut%
  {\setlength{\@xlen}{1.05em}%
   \addtolength{\@xlen}{\pcalvspace}%
    \raisebox{\vshadelen}{\raisebox{-.25em}{\rule{0pt}{\@xlen}}}%
   \global\setlength{\vshadelen}{0pt}%
   \global\setlength{\pcalvspace}{0pt}}

\renewcommand{\@x}[1]{\par
  \ifpcaltlashading
  \makebox[0pt][l]{\shadebox{\xtstrut\hspace*{\textwidth}}}%
  \fi
  \mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}}  

% \@xx{txt} continues a specification line with the text txt.
\renewcommand{\@xx}[1]{\mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}}  

% \@y{cmt} produces a one-line comment.
\renewcommand{\@y}[1]{\mbox{\footnotesize\footnotesize\hspace{.65em}%
  \ifthenelse{\boolean{tlashading}}{%
      \shadebox{#1\hspace{-\the\lastskip}\rstrut}}%
               {#1\hspace{-\the\lastskip}\rstrut}}}

% \@yy{cmt} produces a one-line comment with no additional pre-hspace
\newcommand{\@yy}[1]{\mbox{\footnotesize\footnotesize%
  \ifthenelse{\boolean{tlashading}}{%
      \shadebox{#1\hspace{-\the\lastskip}\rstrut}}%
               {#1\hspace{-\the\lastskip}\rstrut}}}

% \@z{cmt} produces a zero-width one-line comment.
\renewcommand{\@z}[1]{\makebox[0pt][l]{\footnotesize
  \ifthenelse{\boolean{tlashading}}{%
      \shadebox{#1\hspace{-\the\lastskip}\rstrut}}%
               {#1\hspace{-\the\lastskip}\rstrut}}}


% \@w{str} produces the TLA+ string "str".
\renewcommand{\@w}[1]{\textcolor{blue}{{\textsf{``{#1}''}}             }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tlashading                                                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\graymargin{1}
  % The number of points of margin in the shaded box.

% \definecolor{boxshade}{gray}{.85}
% Defines the darkness of the tlashading: 1 = white, 0 = black
% Added by TLATeX only if needed.

% \shadebox{txt} puts txt in a shaded box.
\renewcommand{\shadebox}[1]{{\setlength{\fboxsep}{\graymargin pt}%
     \savebox{\tempboxa}{#1}%
     \settoheight{\templena}{\usebox{\tempboxa}}%
     \settodepth{\templenb}{\usebox{\tempboxa}}%
     \hspace*{-\fboxsep}\raisebox{0pt}[\templena][\templenb]%
        {\colorbox{boxshade}{\usebox{\tempboxa}}}\hspace*{-\fboxsep}}}

% \vshade{n} makes an n-point inter-paragraph space, with
%  tlashading if the `tlashading' flag is true.
\setlength{\vshadelen}{0pt}
\renewcommand{\vshade}[1]{\ifthenelse{\boolean{tlashading}}%
   {\global\setlength{\vshadelen}{#1pt}}%
   {\vspace{#1pt}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE cpar ENVIRONMENT                                                      %
% ^^^^^^^^^^^^^^^^^^^^                                                      %
% The LaTeX input                                                           %
%                                                                           %
%   \begin{cpar}{pop}{nest}{isLabel}{d}{e}{arg6}                            %
%     XXXXXXXXXXXXXXX                                                       %
%     XXXXXXXXXXXXXXX                                                       %
%     XXXXXXXXXXXXXXX                                                       %
%   \end{cpar}                                                              %
%                                                                           %
% produces one of two possible results.  If isLabel is the letter "T",      %
% it produces the following, where [label] is the result of typesetting     %
% arg6 in an LR box, and d is is a number representing a distance in        %
% points.                                                                   %
%                                                                           %
%   prevailing |<-- d -->[label]<- e ->XXXXXXXXXXXXXXX                      %
%         left |                       XXXXXXXXXXXXXXX                      %
%       margin |                       XXXXXXXXXXXXXXX                      %
%                                                                           %
% If isLabel is the letter "F", then it produces                            %
%                                                                           %
%   prevailing |<-- d -->XXXXXXXXXXXXXXXXXXXXXXX                            %
%         left |         <- e ->XXXXXXXXXXXXXXXX                            %
%       margin |                XXXXXXXXXXXXXXXX                            %
%                                                                           %
% where d and e are numbers representing distances in points.               %
%                                                                           %
% The prevailing left margin is the one in effect before the most recent    %
% pop (argument 1) cpar environments with "T" as the nest argument, where   %
% pop is a number \geq 0.                                                   %
%                                                                           %
% If the nest argument is the letter "T", then the prevailing left          %
% margin is moved to the left of the second (and following) lines of        %
% X's.  Otherwise, the prevailing left margin is left unchanged.            %
%                                                                           %
% An \unnest{n} command moves the prevailing left margin to where it was    %
% before the most recent n cpar environments with "T" as the nesting        %
% argument.                                                                 %
%                                                                           %
% The environment leaves no vertical space above or below it, or between    %
% its paragraphs.  (TLATeX inserts the proper amount of vertical space.)    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setcounter{pardepth}{0}

% \setgmargin{txt} defines \gmarginN to be txt, where N is \roman{pardepth}.
% \thegmargin equals \gmarginN, where N is \roman{pardepth}.
\renewcommand{\setgmargin}[1]{%
  \expandafter\xdef\csname gmargin\roman{pardepth}\endcsname{#1}}
\renewcommand{\thegmargin}{\csname gmargin\roman{pardepth}\endcsname}
\renewcommand{\gmargin}{0pt}

%\newlength{\@cparht}
%\newlength{\@cpardp}
\renewenvironment{cpar}[6]{%
  \addtocounter{pardepth}{-#1}%
  \ifthenelse{\boolean{tlashading}}{\par\begin{lrbox}{\tempsbox}%
                                 \begin{minipage}[t]{\linewidth}}{}%
  \begin{list}{}{%
     \edef\temp{\thegmargin}
     \ifthenelse{\equal{#3}{T}}%
       {\settowidth{\leftmargin}{\hspace{\temp}\footnotesize #6\hspace{#5pt}}%
        \addtolength{\leftmargin}{#4pt}}%
       {\setlength{\leftmargin}{#4pt}%
        \addtolength{\leftmargin}{#5pt}%
        \addtolength{\leftmargin}{\temp}%
        \setlength{\itemindent}{-#5pt}}%
      \ifthenelse{\equal{#2}{T}}{\addtocounter{pardepth}{1}%
                                 \setgmargin{\the\leftmargin}}{}%
      \setlength{\labelwidth}{0pt}%
      \setlength{\labelsep}{0pt}%
      \setlength{\itemindent}{-\leftmargin}%
      \setlength{\topsep}{0pt}%
      \setlength{\parsep}{0pt}%
      \setlength{\partopsep}{0pt}%
      \setlength{\parskip}{0pt}%
      \setlength{\itemsep}{0pt}
      \setlength{\itemindent}{#4pt}%
      \addtolength{\itemindent}{-\leftmargin}}%
   \ifthenelse{\equal{#3}{T}}%
      {\item[\tstrut\footnotesize \hspace{\temp}{#6}\hspace{#5pt}]
        }%
      {\item[\tstrut\hspace{\temp}]%
         }%
   \footnotesize}
 {\hspace{-\the\lastskip}\tstrut
 \end{list}%
  \ifthenelse{\boolean{tlashading}}%
          {\end{minipage}%
           \end{lrbox}%
           \ifpcaltlashading
             \setlength{\@cparht}{\ht\tempsbox}%
             \setlength{\@cpardp}{\dp\tempsbox}%
             \addtolength{\@cparht}{.15em}%
             \addtolength{\@cpardp}{.2em}%
             \addtolength{\@cparht}{\@cpardp}%
            % I don't know what's going on here.  I want to add a
            % \pcalvspace high shaded line, but I don't know how to
            % do it.  A little trial and error shows that the following
            % does a reasonable job approximating that, eliminating
            % the line if \pcalvspace is small.
            \addtolength{\@cparht}{\pcalvspace}%
             \ifdim \pcalvspace > .8em
               \addtolength{\pcalvspace}{-.2em}%
               \hspace*{-\lcomindent}%
               \shadebox{\rule{0pt}{\pcalvspace}\hspace*{\textwidth}}\par
               \global\setlength{\pcalvspace}{0pt}%
               \fi
             \hspace*{-\lcomindent}%
             \makebox[0pt][l]{\raisebox{-\@cpardp}[0pt][0pt]{%
                 \shadebox{\rule{0pt}{\@cparht}\hspace*{\textwidth}}}}%
             \hspace*{\lcomindent}\usebox{\tempsbox}%
             \par
           \else
             \shadebox{\usebox{\tempsbox}}\par
           \fi}%
           {}%
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE ppar ENVIRONMENT                                                       %
% ^^^^^^^^^^^^^^^^^^^^                                                       %
% The environment                                                            %
%                                                                            %
%   \begin{ppar} ... \end{ppar}                                              %
%                                                                            %
% is equivalent to                                                           %
%                                                                            %
%   \begin{cpar}{0}{F}{F}{0}{0}{} ... \end{cpar}                             %
%                                                                            %
% The environment is put around each line of the output for a PlusCal        %
% algorithm.                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{ppar}{%
%  \ifthenelse{\boolean{tlashading}}{\par\begin{lrbox}{\tempsbox}%
%                                 \begin{minipage}[t]{\linewidth}}{}%
%  \begin{list}{}{%
%     \edef\temp{\thegmargin}
%        \setlength{\leftmargin}{0pt}%
%        \addtolength{\leftmargin}{\temp}%
%        \setlength{\itemindent}{0pt}%
%      \setlength{\labelwidth}{0pt}%
%      \setlength{\labelsep}{0pt}%
%      \setlength{\itemindent}{-\leftmargin}%
%      \setlength{\topsep}{0pt}%
%      \setlength{\parsep}{0pt}%
%      \setlength{\partopsep}{0pt}%
%      \setlength{\parskip}{0pt}%
%      \setlength{\itemsep}{0pt}
%      \setlength{\itemindent}{0pt}%
%      \addtolength{\itemindent}{-\leftmargin}}%
%      \item[\tstrut\hspace{\temp}]}%
% {\hspace{-\the\lastskip}\tstrut
% \end{list}%
%  \ifthenelse{\boolean{tlashading}}{\end{minipage}  
%                                 \end{lrbox}%
%                                 \shadebox{\usebox{\tempsbox}}\par}{}%
%  }

 %%% TESTING
 \renewcommand{\xtest}[1]{\par
 \makebox[0pt][l]{\shadebox{\xtstrut\hspace*{\textwidth}}}%
 \mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}} 

% \renewcommand{\xxtest}[1]{\par
% \makebox[0pt][l]{\shadebox{\xtstrut{#1}\hspace*{\textwidth}}}%
% \mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}} 

%\newlength{\pcalvspace}
%\setlength{\pcalvspace}{0pt}
% \newlength{\xxtestlen}
% \setlength{\xxtestlen}{0pt}
% \renewcommand\xtstrut%
%   {\setlength{\xxtestlen}{1.15em}%
%    \addtolength{\xxtestlen}{\pcalvspace}%
%     \raisebox{\vshadelen}{\raisebox{-.25em}{\rule{0pt}{\xxtestlen}}}%
%    \global\setlength{\vshadelen}{0pt}%
%    \global\setlength{\pcalvspace}{0pt}}
   
   %%%% TESTING
   
   %% The xcpar environment
   %%  Note: overloaded use of \pcalvspace for testing.
   %%
%   \newlength{\xcparht}%
%   \newlength{\xcpardp}%
   
%   \newenvironment{xcpar}[6]{%
%  \addtocounter{pardepth}{-#1}%
%  \ifthenelse{\boolean{tlashading}}{\par\begin{lrbox}{\tempsbox}%
%                                 \begin{minipage}[t]{\linewidth}}{}%
%  \begin{list}{}{%
%     \edef\temp{\thegmargin}%
%     \ifthenelse{\equal{#3}{T}}%
%       {\settowidth{\leftmargin}{\hspace{\temp}\footnotesize #6\hspace{#5pt}}%
%        \addtolength{\leftmargin}{#4pt}}%
%       {\setlength{\leftmargin}{#4pt}%
%        \addtolength{\leftmargin}{#5pt}%
%        \addtolength{\leftmargin}{\temp}%
%        \setlength{\itemindent}{-#5pt}}%
%      \ifthenelse{\equal{#2}{T}}{\addtocounter{pardepth}{1}%
%                                 \setgmargin{\the\leftmargin}}{}%
%      \setlength{\labelwidth}{0pt}%
%      \setlength{\labelsep}{0pt}%
%      \setlength{\itemindent}{-\leftmargin}%
%      \setlength{\topsep}{0pt}%
%      \setlength{\parsep}{0pt}%
%      \setlength{\partopsep}{0pt}%
%      \setlength{\parskip}{0pt}%
%      \setlength{\itemsep}{0pt}%
%      \setlength{\itemindent}{#4pt}%
%      \addtolength{\itemindent}{-\leftmargin}}%
%   \ifthenelse{\equal{#3}{T}}%
%      {\item[\xtstrut\footnotesize \hspace{\temp}{#6}\hspace{#5pt}]%
%        }%
%      {\item[\xtstrut\hspace{\temp}]%
%         }%
%   \footnotesize}
% {\hspace{-\the\lastskip}\tstrut
% \end{list}%
%  \ifthenelse{\boolean{tlashading}}{\end{minipage}  
%                                 \end{lrbox}%
%                                 \setlength{\xcparht}{\ht\tempsbox}%
%                                 \setlength{\xcpardp}{\dp\tempsbox}%
%                                 \addtolength{\xcparht}{.15em}%
%                                 \addtolength{\xcpardp}{.2em}%
%                                 \addtolength{\xcparht}{\xcpardp}%
%                                 \hspace*{-\lcomindent}%
%                                 \makebox[0pt][l]{\raisebox{-\xcpardp}[0pt][0pt]{%
%                                      \shadebox{\rule{0pt}{\xcparht}\hspace*{\textwidth}}}}%
%                                 \hspace*{\lcomindent}\usebox{\tempsbox}%
%                                 \par}{}%
%  }
%  
% \newlength{\xmcomlen}
%\newenvironment{xmcom}[1]{%
%  \setcounter{pardepth}{0}%
%  \hspace{.65em}%
%  \begin{lrbox}{\alignbox}\sloppypar%
%      \setboolean{tlashading}{true}%
%      \setlength{\boxwidth}{#1pt}%
%      \addtolength{\boxwidth}{-.65em}%
%      \begin{minipage}[t]{\boxwidth}\footnotesize
%      \parskip=0pt\relax}%
%       {\end{minipage}\end{lrbox}%
%       \setlength{\xmcomlen}{\textwidth}%
%       \addtolength{\xmcomlen}{-\wd\alignbox}%
%       \settodepth{\alignwidth}{\usebox{\alignbox}}%
%       \global\setlength{\multicommentdepth}{\alignwidth}%
%       \setlength{\boxwidth}{\alignwidth}%
%       \global\addtolength{\alignwidth}{-\maxdepth}%
%       \addtolength{\boxwidth}{.1em}%
%       \raisebox{0pt}[0pt][0pt]{%
%        \ifthenelse{\boolean{tlashading}}%
%          {\hspace*{-\xmcomlen}\shadebox{\rule[-\boxwidth]{0pt}{0pt}%
%                                 \hspace*{\xmcomlen}\usebox{\alignbox}}}%
%          {\usebox{\alignbox}}}%
%       \vspace*{\alignwidth}\pagebreak[0]\vspace{-\alignwidth}\par}
% % a multi-line comment, whose first argument is its width in points.
%  
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE lcom ENVIRONMENT                                                       %
% ^^^^^^^^^^^^^^^^^^^^                                                       %
% A multi-line comment with no text to its left is typeset in an lcom        % 
% environment, whose argument is a number representing the indentation       % 
% of the left margin, in points.  All the text of the comment should be      % 
% inside cpar environments.                                                  % 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewenvironment{lcom}[1]{%
  \setlength{\lcomindent}{#1pt} % Added for PlusCal handling.
  \par\vspace{.2em}%
  \sloppypar
  \setcounter{pardepth}{0}%
  \footnotesize
  \begin{list}{}{%
    \setlength{\leftmargin}{#1pt}
    \setlength{\labelwidth}{0pt}%
    \setlength{\labelsep}{0pt}%
    \setlength{\itemindent}{0pt}%
    \setlength{\topsep}{0pt}%
    \setlength{\parsep}{0pt}%
    \setlength{\partopsep}{0pt}%
    \setlength{\parskip}{0pt}}
    \item[]}%
  {\end{list}\vspace{.3em}\setlength{\lcomindent}{0pt}%
 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE mcom ENVIRONMENT AND \mutivspace COMMAND                              %
% ^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^                              %
%                                                                           %
% A part of the spec containing a right-comment of the form                 %
%                                                                           %
%      xxxx (*************)                                                 %
%      yyyy (* ccccccccc *)                                                 %
%      ...  (* ccccccccc *)                                                 %
%           (* ccccccccc *)                                                 %
%           (* ccccccccc *)                                                 %
%           (*************)                                                 %
%                                                                           %
% is typeset by                                                             %
%                                                                           %
%     XXXX \begin{mcom}{d}                                                  %
%            CCCC ... CCC                                                   %
%          \end{mcom}                                                       %
%     YYYY ...                                                              %
%     \multivspace{n}                                                       %
%                                                                           %
% where the number d is the width in points of the comment, n is the        %
% number of xxxx, yyyy, ...  lines to the left of the comment.              %
% All the text of the comment should be typeset in cpar environments.       %
%                                                                           %
% This puts the comment into a single box (so no page breaks can occur      %
% within it).  The entire box is shaded iff the tlashading flag is true.       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewenvironment{mcom}[1]{%
  \setcounter{pardepth}{0}%
  \hspace{.65em}%
  \begin{lrbox}{\alignbox}\sloppypar%
      \setboolean{tlashading}{true}%
      \setlength{\boxwidth}{#1pt}%
      \addtolength{\boxwidth}{-.65em}%
      \begin{minipage}[t]{\boxwidth}\footnotesize
      \parskip=0pt\relax}%
       {\end{minipage}\end{lrbox}%
       \setlength{\xmcomlen}{\textwidth}%       % For PlusCal tlashading
       \addtolength{\xmcomlen}{-\wd\alignbox}%  % For PlusCal tlashading
       \settodepth{\alignwidth}{\usebox{\alignbox}}%
       \global\setlength{\multicommentdepth}{\alignwidth}%
       \setlength{\boxwidth}{\alignwidth}%      % For PlusCal tlashading
       \global\addtolength{\alignwidth}{-\maxdepth}%
       \addtolength{\boxwidth}{.1em}%           % For PlusCal tlashading
      \raisebox{0pt}[0pt][0pt]{%
        \ifthenelse{\boolean{tlashading}}%
          {\ifpcaltlashading
             \hspace*{-\xmcomlen}%
             \shadebox{\rule[-\boxwidth]{0pt}{0pt}\hspace*{\xmcomlen}%
                          \usebox{\alignbox}}%
           \else
             \shadebox{\usebox{\alignbox}}
           \fi
          }%
          {\usebox{\alignbox}}}%
       \vspace*{\alignwidth}\pagebreak[0]\vspace{-\alignwidth}\par}
 % a multi-line comment, whose first argument is its width in points.


% \multispace{n} produces the vertical space indicated by "|"s in 
% this situation
%   
%     xxxx (*************)
%     xxxx (* ccccccccc *)
%      |   (* ccccccccc *)
%      |   (* ccccccccc *)
%      |   (* ccccccccc *)
%      |   (*************)
%
% where n is the number of "xxxx" lines.
\renewcommand{\multivspace}[1]{\addtolength{\multicommentdepth}{-#1\baselineskip}%
 \addtolength{\multicommentdepth}{1.2em}%
 \ifthenelse{\lengthtest{\multicommentdepth > 0pt}}%
    {\par\vspace{\multicommentdepth}\par}{}}

%\newenvironment{hpar}[2]{%
%  \begin{list}{}{\setlength{\leftmargin}{#1pt}%
%                 \addtolength{\leftmargin}{#2pt}%
%                 \setlength{\itemindent}{-#2pt}%
%                 \setlength{\topsep}{0pt}%
%                 \setlength{\parsep}{0pt}%
%                 \setlength{\partopsep}{0pt}%
%                 \setlength{\parskip}{0pt}%
%                 \addtolength{\labelsep}{0pt}}%
%  \item[]\footnotesize}{\end{list}}
%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    % Typesets a sequence of paragraphs like this:                         %
%    %                                                                      %
%    %      left |<-- d1 --> XXXXXXXXXXXXXXXXXXXXXXXX                       %
%    %    margin |           <- d2 -> XXXXXXXXXXXXXXX                       %
%    %           |                    XXXXXXXXXXXXXXX                       %
%    %           |                                                          %
%    %           |                    XXXXXXXXXXXXXXX                       %
%    %           |                    XXXXXXXXXXXXXXX                       %
%    %                                                                      %
%    % where d1 = #1pt and d2 = #2pt, but with no vspace between            %
%    % paragraphs.                                                          %
%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands for repeated characters that produce dashes.              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \raisedDash{wd}{ht}{thk} makes a horizontal line wd characters wide, 
% raised a distance ht ex's above the baseline, with a thickness of 
% thk em's.
\renewcommand{\raisedDash}[3]{\raisebox{#2ex}{\setlength{\alignwidth}{.5em}%
  \rule{#1\alignwidth}{#3em}}}

% The following commands take a single argument n and produce the
% output for n repeated characters, as follows
%   \cdash:    -
%   \tdash:    ~
%   \ceqdash:  =
%   \usdash:   _
\renewcommand{\cdash}[1]{\raisedDash{#1}{.5}{.04}}
\renewcommand{\usdash}[1]{\raisedDash{#1}{0}{.04}}
\renewcommand{\ceqdash}[1]{\raisedDash{#1}{.5}{.08}}
\renewcommand{\tdash}[1]{\raisedDash{#1}{1}{.08}}

\setlength{\spacewidth}{.2em}
\renewcommand{\e}[1]{\hspace{#1\spacewidth}}
%% \e{i} produces space corresponding to i input spaces.


%% Alignment-file Commands
% \al{i}{j}{txt} is used in the alignment file to put "%{i}{j}{wd}"
% in the log file, where wd is the width of the line up to that point,
% and txt is the following text.
\renewcommand{\al}[3]{%
  \typeout{\%{#1}{#2}{\the\alignwidth}}%
  \cl{#3}}

%% \cl{txt} continues a specification line in the alignment file
%% with text txt.
\renewcommand{\cl}[1]{%
  \savebox{\alignbox}{\mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}}%
  \settowidth{\alignboxwidth}{\usebox{\alignbox}}%
  \addtolength{\alignwidth}{\alignboxwidth}%
  \usebox{\alignbox}}

% \fl{txt} in the alignment file begins a specification line that
% starts with the text txt.
\renewcommand{\fl}[1]{%
  \par
  \savebox{\alignbox}{\mbox{\footnotesize$\mbox{\footnotesize}#1\mbox{\footnotesize}$}}%
  \settowidth{\alignwidth}{\usebox{\alignbox}}%
  \usebox{\alignbox}}

\makeatletter
\newcommand{\tlx@c}{\c@tlx@ctr\advance\c@tlx@ctr\@ne}
\newcounter{tlx@ctr}
\c@tlx@ctr=\itfam \multiply\c@tlx@ctr"100\relax \advance\c@tlx@ctr "7061\relax
\mathcode`a=\tlx@c \mathcode`b=\tlx@c \mathcode`c=\tlx@c \mathcode`d=\tlx@c
\mathcode`e=\tlx@c \mathcode`f=\tlx@c \mathcode`g=\tlx@c \mathcode`h=\tlx@c
\mathcode`i=\tlx@c \mathcode`j=\tlx@c \mathcode`k=\tlx@c \mathcode`l=\tlx@c
\mathcode`m=\tlx@c \mathcode`n=\tlx@c \mathcode`o=\tlx@c \mathcode`p=\tlx@c
\mathcode`q=\tlx@c \mathcode`r=\tlx@c \mathcode`s=\tlx@c \mathcode`t=\tlx@c
\mathcode`u=\tlx@c \mathcode`v=\tlx@c \mathcode`w=\tlx@c \mathcode`x=\tlx@c
\mathcode`y=\tlx@c \mathcode`z=\tlx@c
\c@tlx@ctr=\itfam \multiply\c@tlx@ctr"100\relax \advance\c@tlx@ctr "7041\relax
\mathcode`A=\tlx@c \mathcode`B=\tlx@c \mathcode`C=\tlx@c \mathcode`D=\tlx@c
\mathcode`E=\tlx@c \mathcode`F=\tlx@c \mathcode`G=\tlx@c \mathcode`H=\tlx@c
\mathcode`I=\tlx@c \mathcode`J=\tlx@c \mathcode`K=\tlx@c \mathcode`L=\tlx@c
\mathcode`M=\tlx@c \mathcode`N=\tlx@c \mathcode`O=\tlx@c \mathcode`P=\tlx@c
\mathcode`Q=\tlx@c \mathcode`R=\tlx@c \mathcode`S=\tlx@c \mathcode`T=\tlx@c
\mathcode`U=\tlx@c \mathcode`V=\tlx@c \mathcode`W=\tlx@c \mathcode`X=\tlx@c
\mathcode`Y=\tlx@c \mathcode`Z=\tlx@c
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                THE describe ENVIRONMENT                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
% It is like the description environment except it takes an argument
% ARG that should be the text of the widest label.  It adjusts the
% indentation so each item with label LABEL produces
%%      LABEL             blah blah blah
%%      <- width of ARG ->blah blah blah
%%                        blah blah blah
\newenvironment{describe}[1]%
   {\begin{list}{}{\settowidth{\labelwidth}{#1}%
            \setlength{\labelsep}{.5em}%
            \setlength{\leftmargin}{\labelwidth}% 
            \addtolength{\leftmargin}{\labelsep}%
            \addtolength{\leftmargin}{\parindent}%
            \def\makelabel##1{\rm ##1\hfill}}%
            \setlength{\topsep}{0pt}}%% 
                % Sets \topsep to 0 to reduce vertical space above
                % and below embedded displayed equations
   {\end{list}}

%   For tlatex.TeX
\makeatletter
\def\tla{\let\%\relax%
         \@bsphack
         \typeout{\%{\the\linewidth}}%
             \let\do\@makeother\dospecials\catcode`\^^M\active
             \let\verbatim@startline\relax
             \let\verbatim@addtoline\@gobble
             \let\verbatim@processline\relax
             \let\verbatim@finish\relax
             \verbatim@}
\let\endtla=\@esphack

\let\pcal=\tla
\let\endpcal=\endtla
\let\ppcal=\tla
\let\endppcal=\endtla

% The tlatex environment is used by TLATeX.TeX to typeset TLA+.
% TLATeX.TLA starts its files by writing a \tlatex command.  This
% command/environment sets \parindent to 0 and defines \% to its
% standard definition because the writing of the log files is messed up
% if \% is defined to be something else.  It also executes
% \@computerule to determine the dimensions for the TLA horizonatl
% bars.
\renewenvironment{tlatex}{\@computerule%
                        \setlength{\parindent}{0pt}%
                       \makeatletter\chardef\%=`\%}{}


% The notla environment produces no output.  You can turn a 
% tla environment to a notla environment to prevent tlatex.TeX from
% re-formatting the environment.

\def\notla{\let\%\relax%
         \@bsphack
             \let\do\@makeother\dospecials\catcode`\^^M\active
             \let\verbatim@startline\relax
             \let\verbatim@addtoline\@gobble
             \let\verbatim@processline\relax
             \let\verbatim@finish\relax
             \verbatim@}
\let\endnotla=\@esphack

\let\nopcal=\notla
\let\endnopcal=\endnotla
\let\noppcal=\notla
\let\endnoppcal=\endnotla

%%%%%%%%%%%%%%%%%%%%%%%% end of tlatex.sty file %%%%%%%%%%%%%%%%%%%%%%% 
% last modified on Fri  3 August 2012 at 14:23:49 PST by lamport

\tlatex
\@x{}\moduleLeftDash\@xx{ {\MODULE} MultiPaxos}\moduleRightDash\@xx{}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
This is a specification in TLA+ and machine checked proof in TLAPS of
Multi-Paxos with Preemption.
\end{cpar}%
\end{lcom}%

%P, A, Q, V  Sets of proposers, acceptors, quorums of acceptors, values to propose
%msgs, pBal, aBal, aVoted
%vote v for s in/with b; vote <b,s,v>
\@x{ {\EXTENDS} Integers ,\, TLAPS ,\, FiniteSets ,\, FiniteSetTheorems}%
\@x{ {\CONSTANTS} {\mathcal{P}} ,\, {\mathcal{A}} ,\, {\mathcal{Q}} ,\, {\mathcal{V}} \@s{17.75}}%
\@y{\@s{0.0}%
 Sets of proposers, acceptors, quorums of acceptors, and values to propose
}%
\@pvspace{8.0pt}%

\@x{ {\VARIABLES} msgs ,\,\@s{10.93}}%
\@y{\@s{0.0}%
 Set of sent messages
}%
\@xx{}%
\@x{\@s{41.14} pBal ,\,\@s{11.67}}%
\@y{\@s{0.0}%
 For each proposer, the current ballot of the proposer
}%
\@xx{}%
\@x{\@s{41.14} aBal ,\,\@s{11.67}}%
\@y{\@s{0.0}%
 For each acceptor, the highest ballot seen by the acceptor
}%
\@xx{}%
\@x{\@s{41.14} aVoted \,\@s{7.35}}%
\@y{\@s{0.0}%
 For each acceptor, a subset of \ensuremath{{\langle}ballot,\, slot,\, value{\rangle}} triples that the acceptor has voted %\ensuremath{VotedForIn} %annie: not use as it is not yet defined
}
\@pvspace{0.0pt}%
%\@x{\@s{75.75}}%
%\@y{\@s{0.0}%
%For every slot voted in, the acceptor only stores the triple with the highest ballot
%}%
\@xx{}%
\@x{ {\ASSUME} QuorumAssumption \.{\defeq} {\mathcal{Q}} \.{\subseteq} {\SUBSET}
 {\mathcal{A}} \.{\land} \A\, Q1 ,\, Q2 \.{\in} {\mathcal{Q}} \.{:} Q1 \.{\cap} Q2
 \.{\neq} {\emptyset}}%
\@pvspace{8.0pt}%
\@x{ {\mathcal{B}} \.{\defeq} {\mathds{N}}\@s{9.5}}%
\@y{\@s{0.0}%
 Set of ballots
}%
\@xx{}%
\@x{ {\mathcal{S}} \.{\defeq} {\mathds{N}}\@s{10}}%
\@y{\@s{0.0}%
 Set of slots
}%
\@xx{}%
\@x{ vars \.{\defeq} {\langle} msgs ,\, pBal ,\, aBal ,\, aVoted {\rangle}}%
\@x{ Send ( m ) \.{\defeq} msgs \.{'} \.{=} msgs \.{\cup} \{ m \}}%
\@pvspace{8.0pt}%
%\begin{lcom}{0}%
%\begin{cpar}{0}{F}{F}{0}{0}{}%
%Following is the specification of the phases of \textit{Multi-Paxos}. These are described in Section~\ref{secSpec}.
%\end{cpar}%
%\end{lcom}%

\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 Phase \ensuremath{1a}: For a proposer \ensuremath{p}, this phase selects some ballot number \ensuremath{pBal[p]} with which
 a \textsf{1a} message has not been sent,
 %This number is sent to any set of acceptors which contains at least one quorum from \ensuremath{{\mathcal{Q}}}.
 %Trivially it can be broadcast 
 and sends it (to all processes). 
 %For safety, any subset of
 %\ensuremath{{\mathcal{A}}} would suffice. For liveness, a subset containing at least one
 %quorum is needed.
\end{cpar}%
\end{lcom}%
 \@x{ Phase1a ( p ) \.{\defeq} \.{\land} {\nexists}\, m \.{\in} msgs \.{:}  m
 . type \.{=}\@w{1a}  \.{\land}  m . bal \.{=} pBal [ p ] }%
 \@x{\@s{55.78} \.{\land} Send ( [ type \.{\mapsto}\@w{1a} ,\, from
 \.{\mapsto} p ,\, bal \.{\mapsto} pBal [ p ] ] )}%
 \@x{\@s{55.78} \.{\land} {\UNCHANGED} {\langle} pBal ,\, aBal ,\, aVoted
 {\rangle}}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 Phase \ensuremath{1b}: For an acceptor \ensuremath{a}, if there is
 a \textsf{1a} message \ensuremath{m} with
 ballot \ensuremath{m.bal} that is
 %than that of any \textsf{1a} message to which it has already responded,
 higher than the highest it has seen, % \ensuremath{aBal[a]}, then
 \ensuremath{a} sends a \textsf{1b} message with \ensuremath{m.bal} and with the set of highest-numbered triples it has voted for each slot, and it updates the highest ballot it has seen to be $m.bal$;
 %a promise, that is a \textsf{1b} message, not to accept any more proposals
 %for ballots numbered less than \ensuremath{m.bal} by updating its \ensuremath{aBal} to \ensuremath{m.bal}; 
 otherwise it sends a \textsf{preempt} message
back with the highest ballot it has seen.
 %In case of a \textsf{1b} reply, the acceptor writes a mapping in
 %\ensuremath{{\mathcal{S}} \.{\rightarrow}
 %{\mathcal{B}} \.{\times} {\mathcal{V}}}. This mapping reveals for each slot, the value
 %that the acceptor most recently (that is, highest ballot) voted on, if
 %any. This is maintained in \ensuremath{aVoted}.
 %annie: I think voted are now triples, not S->B x V any more. ?  same to fix in paper body.
\end{cpar}%
\end{lcom}%
 \@x{ Phase1b ( a ) \.{\defeq} \E\, m \.{\in} msgs \.{:} m . type \.{=}\@w{1a}
 \.{\land}}%
\@x{\@s{4.0} {\IF} m . bal \.{>} aBal [ a ] \.{\THEN}}%
 \@x{\@s{13.72} \.{\land} Send ( [ type \.{\mapsto}\@w{1b} ,\, from
 \.{\mapsto} a ,\, bal \.{\mapsto} m . bal ,\, voted \.{\mapsto} aVoted [ a ]
 ] )}%
 \@x{\@s{13.72} \.{\land} aBal \.{'} \.{=} [ aBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
\@x{\@s{13.72} \.{\land} {\UNCHANGED} {\langle} pBal ,\, aVoted {\rangle}}%
\@x{\@s{2.0} \.{\ELSE}}%
 \@x{\@s{10.0} \.{\land} Send ( [ type \.{\mapsto}\@w{preempt} ,\, to
 \.{\mapsto} m . from ,\, bal \.{\mapsto} aBal [ a ] ] )}%
 \@x{\@s{10.0} \.{\land} {\UNCHANGED} {\langle} pBal ,\, aBal ,\, aVoted
 {\rangle}}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 Phase \ensuremath{2a}: For a proposer \ensuremath{p}, 
 if there is no \textsf{2a} message with current ballot \ensuremath{pBal[p]}, and 
 %there is a set \ensuremath{S} of %it receives a response to its \textsf{1a} message (for
 %\textsf{1b} messages with \ensuremath{pBal[p]} such that every acceptor in some quorum has sent some message in \ensuremath{S}, 
 a quorum of acceptors has sent a set \ensuremath{S} of \textsf{1b} messages with \ensuremath{pBal[p]},
 \ensuremath{p} sends a
 \textsf{2a} message %to all acceptors 
 with \ensuremath{pBal[p]} and a set of proposals \ensuremath{PropSV(T)}, where \ensuremath{T} is the union of all voted triples in messages in \ensuremath{S}. \ensuremath{PropSV(T)} includes \ensuremath{MaxSV(T)}, the set of slot-value pairs with the highest ballot for each slot in \ensuremath{T}, and \ensuremath{NewSV(T)}, a set of new slot-value pairs for slots not in \ensuremath{T}.
\end{cpar}%
\end{lcom}%
%notes:
%MaxSV: bmax in FM16, Pmax in vrapaxos, pmax in paxos in da
%MaxBSV: partialMaxSV in proof, max_prop in paxos in da
%UnusedS: Free slots
%NewSV: new props
%PropSV: proposals; for field propSV
 \@x{ MaxBSV ( T )\@s{8.96} \.{\defeq} \{ t \.{\in} T \.{:} \A\, t2
 \.{\in} T \.{:} t2 . slot \.{=} t . slot \.{\implies} t2 . bal \.{\leq} t .
 bal \}}%
 \@x{ MaxSV ( T )\@s{15} \.{\defeq} \{ [ slot \.{\mapsto} t . slot ,\, val
 \.{\mapsto} t . val ] \.{:} t \.{\in} MaxBSV ( T ) \}}%
 \@x{ UnusedS ( T )\@s{12} \.{\defeq} \{ s \.{\in} {\mathcal{S}} \.{:} {\nexists}
 \, t \.{\in} T \.{:} t . slot \.{=} s \}}%
 \@x{ NewSV ( T )\@s{15} \.{\defeq} {\CHOOSE} D \,{\subseteq} [
 slot \,{:} UnusedS ( T ) ,\, val \,{:} {\mathcal{V}} ]
 \,{:} \A\, d1 ,\, d2 \,{\in} D \,{:} d1 . slot \,{=} d2 . slot
 \,{\implies} d1 \,{=} d2 \,{\land} D \, {\neq} \,{\emptyset}}%
\@x{ PropSV ( T )\@s{13} \.{\defeq} MaxSV ( T ) \.{\cup} NewSV ( T )}%
\@pvspace{8.0pt}%
\@x{ Phase2a ( p ) \.{\defeq}}%
 \@x{\@s{4.0} \.{\land} {\nexists}\, m \.{\in} msgs \.{:} ( m . type
 \.{=}\@w{2a} ) \.{\land} ( m . bal \.{=} pBal [ p ] )}%
 \@x{\@s{4.0} \.{\land} \E\, Q \.{\in} {\mathcal{Q}} ,\, S \.{\subseteq} \{ m
 \.{\in} msgs \.{:}  m . type \.{=}\@w{1b}  \.{\land}  m . bal \.{=} pBal
 [ p ]  \} \.{:}}%
 \@x{\@s{16.89} \.{\land} \A\, a \.{\in} Q \.{:} \E\, m \.{\in} S \.{:} m .
 from \.{=} a}%
 \@x{\@s{16.89} \.{\land} Send ( [ type \.{\mapsto}\@w{2a} ,\, from
 \.{\mapsto} p ,\, bal \.{\mapsto} pBal [ p ] ,\, propSV \.{\mapsto}
 PropSV ( {\UNION} \{ m . voted \.{:} m \.{\in} S \} ) ] )}%
 \@x{\@s{4.0} \.{\land} {\UNCHANGED} {\langle} pBal ,\, aBal ,\, aVoted
 {\rangle}}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 Phase \ensuremath{2b}: For an acceptor \ensuremath{a}, if there is a \textsf{2a} message \ensuremath{m} with ballot \ensuremath{m.bal}
 that is higher than or equal to the highest it has seen, \ensuremath{a} 
 %votes for all the message\mbox{\footnotesize'}s values
 %in ballot \ensuremath{m.bal}; 
 sends a \textsf{2b} message with \ensuremath{m.bal} and \ensuremath{m.propSV}, 
 updates the highest ballot it has seen to \ensuremath{m.bal}, and 
 updates set of voted triples using \ensuremath{m.propSV};
 %
 otherwise it sends a \textsf{preempt} message back with the highest ballot it has seen.
\end{cpar}%
\end{lcom}%
 \@x{ Phase2b ( a ) \.{\defeq} \E\, m \.{\in} msgs \.{:} m . type \.{=}\@w{2a}
 \.{\land}}%
\@x{\@s{4.0} {\IF} m . bal \.{\geq} aBal [ a ] \.{\THEN}}%
 \@x{\@s{13.72} \.{\land} Send ( [ type \.{\mapsto}\@w{2b} ,\, from
 \.{\mapsto} a ,\, bal \.{\mapsto} m . bal ,\, propSV \.{\mapsto} m .
 propSV ] )}%
 \@x{\@s{13.72} \.{\land} aBal \.{'} \.{=} [ aBal {\EXCEPT} {\bang} [ a ]
 \.{=} m . bal ]}%
 \@x{\@s{13.72} \.{\land} aVoted \.{'} \.{=} [ aVoted {\EXCEPT} {\bang} [ a ]
 \.{=} \{ [ bal \.{\mapsto} m . bal ,\, slot \.{\mapsto} d . slot ,\,
 val \.{\mapsto} d . val ] \.{:} d \.{\in} m . propSV \} \.{\cup}}%
 \@x{\@s{145.1} \{ e \.{\in} aVoted [ a ] \.{:} {\nexists}\, r \.{\in} m . propSV
 \.{:} e . slot \.{=} r . slot \} ]}%
\@x{\@s{13.72} \.{\land} {\UNCHANGED} {\langle} pBal {\rangle}}%
\@x{\@s{2.0} \.{\ELSE}}%
 \@x{\@s{10.0} \.{\land} Send ( [ type \.{\mapsto}\@w{preempt} ,\, to
 \.{\mapsto} m . from ,\, bal \.{\mapsto} aBal [ a ] ] )}%
 \@x{\@s{10.0} \.{\land} {\UNCHANGED} {\langle} pBal ,\, aBal ,\, aVoted
 {\rangle}}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
Preempt: For a proposer \ensuremath{p}, if there is a \textsf{preempt} message \ensuremath{m} with ballot \ensuremath{m.bal} that is higher than \ensuremath{p}'s current ballot, \ensuremath{p} updates its current ballot to a new ballot that is higher than \ensuremath{m.bal}
 and with which no \textsf{1a} message has been sent.
\end{cpar}%
\end{lcom}%
 \@x{ NewBal ( b2 ) \.{\defeq} {\CHOOSE} b \.{\in} {\mathcal{B}} \.{:} b \.{>} b2
 \.{\land} {\nexists}\, m \.{\in} msgs \.{:} m . type \.{=}\@w{1a} \.{\land}
 m . bal \.{=} b}%
\@x{ Preempt ( p ) \.{\defeq} \E\, m \.{\in} msgs \.{:}}%
 \@x{\@s{4.0} \.{\land} m . type \.{=}\@w{preempt} \.{\land} m . to \.{=} p
 \.{\land} m . bal \.{>} pBal [ p ]}%
 \@x{\@s{4.0} \.{\land} pBal \.{'} \.{=} [ pBal {\EXCEPT} {\bang} [ p ] \.{=}
 NewBal ( m . bal ) ]}%
 \@x{\@s{4.0} \.{\land} {\UNCHANGED} {\langle} msgs ,\, aBal ,\, aVoted
 {\rangle}}%
\@pvspace{8.0pt}%
 \@x{ Init\@s{3.3} \.{\defeq} msgs \.{=} {\emptyset}\@s{2.0} \.{\land} pBal \.{=} [ p \.{\in}
 {\mathcal{P}} \.{\mapsto} 0 ]\@s{2.0} \.{\land} aBal \.{=} [ a \.{\in}
 {\mathcal{A}} \.{\mapsto} \.{-} 1 ]\@s{2.0} \.{\land} aVoted \.{=} [ a \.{\in} {\mathcal{A}} \.{\mapsto}
 {\emptyset} ]}%
 \@x{ Next \.{\defeq} \.{\lor} \E\, p\@s{0.1} \.{\in} {\mathcal{P}} \.{:} Phase1a
 ( p ) \.{\lor} Phase2a ( p ) \.{\lor} Preempt ( p )}%
 \@x{\@s{31.86} \.{\lor} \E\, a \.{\in} {\mathcal{A}}\@s{0.6} \.{:} Phase1b ( a
 )\@s{0.41} \.{\lor} Phase2b ( a )}%
\@x{ Spec\@s{1.17} \.{\defeq} Init \.{\land} {\Box} [ Next ]_{ vars}}%
\@pvspace{8.0pt}%

\@x{}\midbar\@xx{}%
\iffalse
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
How a value is chosen:
%\end{cpar}%
%\vshade{5.0}%
%\begin{cpar}{0}{F}{F}{0}{0}{}%
This spec does not contain any actions in which a value is explicitly
 chosen (or a chosen value learned). What it means for a value to be
 chosen is defined by the operator \ensuremath{Chosen}, where
 \ensuremath{Chosen(s,\, v)} means that
 value \ensuremath{v} has been chosen for slot \ensuremath{s}. These are described in detail in Section~\ref{secAuxiliary}.
\end{cpar}%
\end{lcom}%
\fi
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{VotedForIn(a, b, s, v)} means that acceptor \ensuremath{a} has sent some \textsf{2b} message \ensuremath{m} with \ensuremath{m.bal} equal to \ensuremath{b} and some proposal in \ensuremath{m.propSV} with \ensuremath{slot} equal to \ensuremath{s} and \ensuremath{val} equal to \ensuremath{v}. This specifies that acceptor \ensuremath{a} has voted the triple \ensuremath{\langle b, s, v\rangle}.
\end{cpar}%
\end{lcom}%
\@x{ VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\defeq} \E\, m \.{\in} msgs \.{:}}%
 \@x{\@s{4.0} m . type \.{=}\@w{2b} \.{\land} m . from\@s{0.36} \.{=} a
 \.{\land} m . bal \.{=} b \.{\land} \E\, d \.{\in} m . propSV \.{:} d .
 slot \.{=} s \.{\land} d . val \.{=} v}%

\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{ChosenIn(b, s, v)} means that every acceptor in some quorum \ensuremath{Q} has voted the triple \ensuremath{\langle b, s, v\rangle}.
\end{cpar}%
\end{lcom}%
 \@x{ ChosenIn ( b ,\, s ,\, v ) \.{\defeq} \E\, Q \.{\in} {\mathcal{Q}} \.{:} \A\,
 a \.{\in} Q \.{:} VotedForIn ( a ,\, b ,\, s ,\, v )}%
 
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Chosen(s, v)} means that for some ballot \ensuremath{b}, \ensuremath{ChosenIn(b, s, v)} holds. 
%We define \ensuremath{Safe} property in terms of this operator.
\end{cpar}%
\end{lcom}%
 \@x{ Chosen ( s ,\, v ) \.{\defeq} \E\, b \.{\in} {\mathcal{B}} \.{:} ChosenIn ( b
 ,\, s ,\, v )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \ensuremath{WontVoteIn(a,\, b,\, s)} means that acceptor \ensuremath{a} has seen a higher ballot than \ensuremath{b}, and did not and will not vote 
 any value with \ensuremath{b} for slot \ensuremath{s}.
\end{cpar}%
\end{lcom}%
 \@x{ WontVoteIn ( a ,\, b ,\, s ) \.{\defeq} aBal [ a ] \.{>} b \.{\land}
 \A\, v \.{\in} {\mathcal{V}} \.{:} {\lnot} VotedForIn ( a ,\, b ,\, s ,\, v )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \ensuremath{SafeAt(b,\, s,\, v)} means that no value except perhaps \ensuremath{v} has been or will be chosen in any ballot lower
 than \ensuremath{b} for slot \ensuremath{s}.
\end{cpar}%
\end{lcom}%
 \@x{ SafeAt ( b ,\, s ,\, v ) \.{\defeq} \A\, b2 \.{\in} 0 \.{\dotdot} ( b
 \.{-} 1 ) \.{:} \E\, Q \.{\in} {\mathcal{Q}} \.{:} \A\, a \.{\in} Q \.{:}
 VotedForIn ( a ,\, b2 ,\, s ,\, v ) \.{\lor} WontVoteIn ( a ,\, b2 ,\, s )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Safe} states that at most one value can be chosen for each slot.
\end{cpar}%
\end{lcom}%
 \@x{ Safe \.{\defeq} \A\, v1 ,\, v2 \.{\in} {\mathcal{V}} ,\, s \.{\in} {\mathcal{S}}
 \.{:} Chosen ( s ,\, v1 ) \.{\land} Chosen ( s ,\, v2 ) \.{\implies} v1
 \.{=} v2 }%
\@pvspace{8.0pt}%

\@x{}\midbar\@xx{}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Messages} defines the set of valid messages. % that can be sent in this specification.
\ensuremath{TypeOK} defines invariants for the types of the variables. 
%These are described in detail in Section~\ref{secTypeInv}.
\end{cpar}%
\end{lcom}%
 \@x{ Messages \.{\defeq} [ type \.{:} \{\@w{1a} \} ,\, from\@s{0.29} \.{:}
 {\mathcal{P}} ,\, bal \.{:} {\mathcal{B}} ] \.{\cup}}%
 \@x{\@s{49.3} [ type \.{:} \{\@w{1b} \} ,\, from \.{:} {\mathcal{A}} ,\,
 bal\@s{0.6} \.{:} {\mathcal{B}} ,\, voted \.{:} {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\,
 slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ] \.{\cup}}%
 \@x{\@s{49.3} [ type \.{:} \{\@w{2a} \} ,\, from\@s{0.29} \.{:} {\mathcal{P}}
 ,\, bal \.{:} {\mathcal{B}} ,\, propSV \.{:} {\SUBSET} [ slot \.{:} {\mathcal{S}} ,\,
 val\@s{0.99} \.{:} {\mathcal{V}} ] ] \.{\cup}}%
 \@x{\@s{49.3} [ type \.{:} \{\@w{2b} \} ,\, from \.{:} {\mathcal{A}} ,\,
 bal\@s{0.6} \.{:} {\mathcal{B}} ,\, propSV \.{:} {\SUBSET} [ slot \.{:} {\mathcal{S}}
 ,\, val\@s{0.99} \.{:} {\mathcal{V}} ] ] \.{\cup}}%
 \@x{\@s{49.3} [ type \.{:} \{\@w{preempt} \} ,\, to \.{:} {\mathcal{P}} ,\, bal
 \.{:} {\mathcal{B}} ]}%
 \@x{ TypeOK \.{\defeq} \.{\land} msgs \.{\subseteq} Messages \.{\land} IsFiniteSet ( msgs ) \.{\land} pBal \.{\in} [ {\mathcal{P}}
 \.{\rightarrow} {\mathcal{B}} ]}%
 \@x{\@s{44.5} \.{\land} aBal\@s{0.74} \.{\in} [ {\mathcal{A}} \.{\rightarrow}
 {\mathcal{B}} \.{\cup} \{ \.{-} 1 \} ] \.{\land} aVoted \.{\in} [ {\mathcal{A}} \.{\rightarrow} {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\,
 slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ]}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Max(T)} selects the largest element in nonempty set \ensuremath{T}.
\end{cpar}%
\end{lcom}%
 \@x{ Max ( T ) \.{\defeq} {\CHOOSE} e \.{\in} T \.{:} \A\, f \.{\in} T \.{:}
 e \.{\geq} f}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
% Given a set of records \ensuremath{S} and a slot \ensuremath{s},
\ensuremath{MaxBalInSlot(T,\, s)} 
%selects the highest ballot \ensuremath{b} such that \ensuremath{[bal \mapsto b, slot \mapsto s] \in S}
selects, among set of elements in \ensuremath{T} with slot \ensuremath{s}, the highest ballot, or -1 if no element has slot \ensuremath{s}.
\end{cpar}%
\end{lcom}%
 \@x{ MaxBalInSlot ( T ,\, s ) \.{\defeq} \.{\LET} E \.{\defeq} \{ e \.{\in} T \.{:} e . slot \.{=} s \} \@s{2.0} \.{\IN} \.{\IF} E \.{=} {\emptyset}
 \.{\THEN} \.{-} 1 \.{\ELSE} Max ( \{e.bal \.{:} e \.{\in} E\} )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{MsgInv} defines properties satisfied by the contents of messages, for 1b, 2a, and 2b messages.
%specifies the message invariant, as described in Section~\ref{secMsgInv}. These invariants specify properties satisfied by the content of the messages classified by message types. In this specification we have three types, \ensuremath{1b}, \ensuremath{2a}, and \ensuremath{2b} for which invariants have been specified by predicates \ensuremath{MsgInv1b}, \ensuremath{MsgInv2a}, and \ensuremath{MsgInv2b}.
\end{cpar}%
\end{lcom}%
 \@x{ MsgInv1b ( m )\@s{0.51} \.{\defeq} \.{\land} m . bal \.{\leq} aBal [ m .
 from ]}%
 \@x{\@s{63.75} \.{\land} \A\, r \.{\in} m . voted \.{:} VotedForIn ( m . from
 ,\, r . bal ,\, r . slot ,\, r . val )}%
 \@x{\@s{63.75} \.{\land} \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v
 \.{\in} {\mathcal{V}} \.{:} b \.{\in} MaxBalInSlot ( m . voted ,\, s ) \.{+} 1
 \.{\dotdot} m . bal \.{-} 1 \.{\implies}}%
\@x{\@s{80.1} {\lnot} VotedForIn ( m . from ,\, b ,\, s ,\, v )}%
\@pvspace{8.0pt}%
 \@x{ MsgInv2a ( m ) \.{\defeq} \.{\land} \A\, d \.{\in} m . propSV \.{:}
 SafeAt ( m . bal ,\, d . slot ,\, d . val )}%
 \@x{\@s{63.75} \.{\land} \A\, d1 ,\, d2 \.{\in} m . propSV \.{:} d1 . slot
 \.{=} d2 . slot \.{\implies} d1 \.{=} d2}%
 \@x{\@s{63.75} \.{\land} \A\, m2 \.{\in} msgs \.{:} ( m2 . type \.{=}\@w{2a}
 \.{\land} m2 . bal \.{=} m . bal ) \.{\implies} m2 \.{=} m}%
\@pvspace{8.0pt}%
 \@x{ MsgInv2b ( m )\@s{0.51} \.{\defeq} \.{\land} \E\, m2 \.{\in} msgs \.{:}
 m2 . type \.{=}\@w{2a} \.{\land} m2 . bal \.{=} m . bal \.{\land} m2 .
 propSV \.{=} m . propSV}%
\@x{\@s{63.75} \.{\land} m . bal \.{\leq} aBal [ m . from ]}%
\@pvspace{8.0pt}%
 \@x{ MsgInv \.{\defeq} \A\, m \.{\in} msgs \.{:} \.{\land} ( m . type
 \.{=}\@w{1b} ) \.{\implies} MsgInv1b ( m )}%
 \@x{\@s{90.0} \.{\land} ( m . type \.{=}\@w{2a} )\@s{0.29} \.{\implies}
 MsgInv2a ( m )}%
 \@x{\@s{90.0} \.{\land} ( m . type \.{=}\@w{2b} )\@s{0.29} \.{\implies}
 MsgInv2b ( m )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{AccInv} defines 
%as described in Section~\ref{secAccInv}. These invariants specify 
properties satisfied by the data maintained by the acceptors. % processes throughout execution.
\end{cpar}%
\end{lcom}%
\@x{ AccInv\@s{1.63} \.{\defeq} \A\, a\@s{2.45} \.{\in} {\mathcal{A}} \.{:}}%
 \@x{\@s{4.0} \.{\land} aBal [ a ] \.{=} \.{-} 1 \.{\implies} aVoted [ a ]
 \.{=} {\emptyset}}%
 \@x{\@s{4.0} \.{\land} \A\, r \.{\in} aVoted [ a ] \.{:} aBal [ a ] \.{\geq}
 r . bal \.{\land} VotedForIn ( a ,\, r . bal ,\, r . slot ,\, r . val )}%
 \@x{\@s{4.0} \.{\land} \A\, b\@s{0.05} \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}}
 ,\, v \.{\in} {\mathcal{V}} \.{:} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\implies}
 \E\, r \.{\in} aVoted [ a ] \.{:} r . bal \.{\geq} b \.{\land} r . slot
 \.{=} s}%
 \@x{\@s{4.0} \.{\land} \A\, b\@s{0.05} \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}}
 ,\, v \.{\in} {\mathcal{V}} \.{:} b \.{>} MaxBalInSlot ( aVoted [ a ] ,\, s )
 \.{\implies} {\lnot} VotedForIn ( a ,\, b ,\, s ,\, v )}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Inv} is the complete inductive invariant.
\end{cpar}%
\end{lcom}%
\@x{ Inv \.{\defeq} TypeOK \.{\land} AccInv \.{\land} MsgInv}%
%\@pvspace{8.0pt}%

\@x{}\midbar\@xx{}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
The following 2 axioms and 10 lemmas are straightforward consequences of the predicates defined above. 
\end{cpar}%
\end{lcom}%
 \@x{ {\AXIOM} MaxInSet\@s{4.9} \.{\defeq} \A\, S \.{\in} ( {\SUBSET} {\mathds{N}} )
 \.{\,\backslash\,} {\emptyset} \.{:} Max ( S ) \.{\in} S}%
 \@x{ {\AXIOM} MaxOnNat \.{\defeq} \A\, S \.{\in} {\SUBSET} {\mathds{N}} \.{:} {\nexists}
 \, s \.{\in} S \.{:} Max ( S ) \.{<} s}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxOnNatS \.{\defeq} \A\, S1 ,\, S2 \.{\in} ( {\SUBSET} {\mathds{N}} )
 \.{\,\backslash\,} {\emptyset} \.{:} S1 \.{\subseteq} S2 \.{\implies} Max ( S1 )
 \.{\leq} Max ( S2 )\@s{2.0} {\BY} MaxInSet}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxBinSType \.{\defeq} \A\, S \.{\in} {\SUBSET} [ bal \.{:}
 {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, s \.{\in} {\mathcal{S}}
 \.{:} MaxBalInSlot ( S ,\, s ) \.{\in} {\mathcal{B}} \.{\cup} \{ \.{-} 1 \}}%
\@x{ {\BY} MaxInSet {\DEF} MaxBalInSlot}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxBinSSubsets \.{\defeq} \A\, S1 ,\, S2 \.{\in} {\SUBSET} [ bal
 \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, s \.{\in}
 {\mathcal{S}} \.{:} S1 \.{\subseteq} S2 \.{\implies}}%
 \@x{\@s{95.72} MaxBalInSlot ( S1 ,\, s ) \.{\leq} MaxBalInSlot ( S2
 ,\, s )}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} {\NEW} S1 \.{\in}
 {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]
 ,\, {\NEW} s \.{\in} {\mathcal{S}} ,\,}%
 \@x{\@s{83.25} {\NEW} S2 \.{\in} {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\, slot
 \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, S1 \.{\subseteq} S2}%
 \@x{\@s{52.31} {\PROVE} MaxBalInSlot ( S1 ,\, s ) \.{\leq}
 MaxBalInSlot ( S2 ,\, s ) \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{4.0}\@pfstepnum{1}{1.} {\CASE} {\nexists}\, d \.{\in} S1 \.{:} d .
 slot \.{=} s}%
 \@x{\@s{8.0}\@pfstepnum{2}{1.}\  MaxBalInSlot ( S1 ,\, s ) \.{=} \.{-}
 1\@s{2.0} {\BY}\@pfstepnum{1}{1}\  {\DEF} MaxBalInSlot}%
 \@x{\@s{8.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{1} ,\, MaxBinSType
 {\DEF} {\mathcal{B}}}%
 \@x{\@s{4.0}\@pfstepnum{1}{2.} {\CASE} \E\, d \.{\in} S1 \.{:} d . slot \.{=}
 s}%
 \@x{\@s{8.0}\@pfstepnum{2}{1.} {\CASE} {\nexists}\, d \.{\in} S2
 \.{\,\backslash\,} S1 \.{:} d . slot \.{=} s}%
 \@x{\@s{12.0}\@pfstepnum{3}{1.}\  MaxBalInSlot ( S1 ,\, s ) \.{=}
 MaxBalInSlot ( S2 ,\, s )\@s{2.0} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{1}{2}\  {\DEF} MaxBalInSlot}%
 \@x{\@s{12.0}\@pfstepnum{3}{}\  {\QED} {\BY}\@pfstepnum{3}{1} ,\, MaxBinSType
 {\DEF} {\mathcal{B}}}%
 \@x{\@s{8.0}\@pfstepnum{2}{2.} {\CASE} \E\, d \.{\in} S2 \.{\,\backslash\,}
 S1 \.{:} d . slot \.{=} s\@s{2.0} {\BY}\@pfstepnum{2}{2}
 ,\,\@pfstepnum{1}{2} ,\, MaxBinSType ,\, MaxOnNatS {\DEF} {\mathcal{B}} ,\,
 MaxBalInSlot}%
 \@x{\@s{8.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{2}{2}\ }%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1}
 ,\,\@pfstepnum{1}{2}\ }%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxBinSNoSlot \.{\defeq} \A\, S \.{\in} {\SUBSET} [ bal \.{:}
 {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, s \.{\in} {\mathcal{S}}
 \.{:}}%
 \@x{\@s{93.8} ( {\nexists}\, d \.{\in} S \.{:} d . slot \.{=} s )
 \.{\equiv} MaxBalInSlot ( S ,\, s ) \.{=} \.{-} 1}%
\@x{ {\BY} MaxInSet {\DEF} MaxBalInSlot ,\, {\mathcal{B}}}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxBinSExists \.{\defeq} \A\, S \.{\in} {\SUBSET} [ bal \.{:}
 {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, s \.{\in} {\mathcal{S}}
 \.{:} MaxBalInSlot ( S ,\, s ) \.{\in} {\mathcal{B}} \.{\implies}}%
 \@x{\@s{91.16} \E\, d \.{\in} S \.{:} d . slot \.{=} s \.{\land} d . bal
 \.{=} MaxBalInSlot ( S ,\, s )}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} {\NEW} S \.{\in}
 {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]
 ,\,}%
 \@x{\@s{83.25} {\NEW} s\@s{1.52} \.{\in} {\mathcal{S}} ,\, MaxBalInSlot ( S ,\, s
 ) \.{\in} {\mathcal{B}}}%
 \@x{\@s{52.31} {\PROVE} \E\, d \.{\in} S \.{:} d . bal \.{=}
 MaxBalInSlot ( S ,\, s ) \.{\land} d . slot \.{=} s \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{8.0}\@pfstepnum{1}{1.}\  \E\, d \.{\in} S \.{:} d . slot \.{=}
 s\@s{2.0} {\BY} {\DEF} MaxBalInSlot ,\, {\mathcal{B}}}%
 \@x{\@s{8.0}\@pfstepnum{1}{2.}\  MaxBalInSlot ( S ,\, s ) \.{=} Max ( \{
 d . bal \.{:} d \.{\in} \{ d \.{\in} S \.{:} d . slot \.{=} s \} \}
 )\@s{2.0} {\BY}\@pfstepnum{1}{1}\  {\DEF} MaxBalInSlot}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1}
 ,\,\@pfstepnum{1}{2} ,\, MaxInSet}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} MaxBinSNoMore \.{\defeq} \A\, S \.{\in} {\SUBSET} [ bal \.{:}
 {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\, s \.{\in} {\mathcal{S}}
 \.{:}}%
 \@x{\@s{98.26} {\nexists}\, d \.{\in} S \.{:} d . bal \.{>} MaxBalInSlot
 ( S ,\, s ) \.{\land} d . slot \.{=} s}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} {\NEW} S \.{\in}
 {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]
 ,\, {\NEW} s \.{\in} {\mathcal{S}}}%
 \@x{\@s{52.31} {\PROVE} {\nexists}\, d \.{\in} S \.{:} d . bal \.{>}
 MaxBalInSlot ( S ,\, s ) \.{\land} d . slot \.{=} s \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{8.0}\@pfstepnum{1}{1.} {\CASE} {\nexists}\, d \.{\in} S \.{:} d .
 slot \.{=} s\@s{2.0} {\BY}\@pfstepnum{1}{1}\ }%
 \@x{\@s{8.0}\@pfstepnum{1}{2.} {\CASE} \E\, d \.{\in} S \.{:} d . slot \.{=}
 s}%
 \@x{\@s{12.0}\@pfstepnum{2}{1.}\  {\nexists}\, b \.{\in} \{ d . bal \.{:} d
 \.{\in} \{ d \.{\in} S \.{:} d . slot \.{=} s \} \} \.{:} b \.{>}
 MaxBalInSlot ( S ,\, s )}%
 \@x{\@s{31.1} {\BY}\@pfstepnum{1}{2} ,\, MaxOnNat {\DEF} MaxBalInSlot ,\,
 {\mathcal{B}} ,\, {\mathcal{S}}}%
 \@x{\@s{12.0}\@pfstepnum{2}{2.}\  {\nexists}\, d \.{\in} S \.{:} ( d . slot
 \.{=} s \.{\land} {\lnot} ( d . bal \.{\leq} MaxBalInSlot ( S ,\, s ) )
 )\@s{2.0} {\BY}\@pfstepnum{2}{1}\ }%
\@x{\@s{12.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{2}\ }%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1}
 ,\,\@pfstepnum{1}{2}\ }%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} Misc \.{\defeq} \A\, S \.{:} \@s{1.25} \.{\land} NewSV ( S )
 \.{\in} ( {\SUBSET} [ slot \.{:} UnusedS ( S ) ,\, val \.{:} {\mathcal{V}} ] )
 \.{\,\backslash\,} {\emptyset}}%
 \@x{\@s{79.71} \.{\land} \A\, t1 ,\, t2 \.{\in} NewSV ( S ) \.{:} t1 .
 slot \.{=} t2 . slot \.{\implies} t1 \.{=} t2}%
 \@x{\@s{79.71} \.{\land} {\nexists}\, t1 \.{\in} MaxSV ( S ) ,\, t2 \.{\in}
 NewSV ( S ) \.{:} t1 . slot \.{=} t2 . slot}%
\@x{\@s{4.0}\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} {\NEW} S}%
 \@x{\@s{52.31} {\PROVE}\@s{-1.5} \.{\land} NewSV ( S ) \.{\in} (
 {\SUBSET} [ slot \.{:} UnusedS ( S ) ,\, val \.{:} {\mathcal{V}} ] )
 \.{\,\backslash\,} {\emptyset}}%
 \@x{\@s{81.63} \.{\land} \A\, t1 ,\, t2 \.{\in} NewSV ( S ) \.{:} t1
 . slot \.{=} t2 . slot \.{\implies} t1 \.{=} t2}%
 \@x{\@s{81.63} \.{\land} {\nexists}\, t1 \.{\in} MaxSV ( S ) ,\, t2 \.{\in}
 NewSV ( S ) \.{:} t1 . slot \.{=} t2 . slot \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{4.0}\@pfstepnum{1}{1.}\  \E\, T \.{\in} ( {\SUBSET} [ slot \.{:}
 UnusedS ( S ) ,\, val \.{:} {\mathcal{V}} ] ) \.{\,\backslash\,} {\emptyset} \.{:} \A\,
 t1 ,\, t2 \.{\in} T \.{:} t1 . slot \.{=} t2 . slot \.{\implies} t1 \.{=}
 t2}%
\@x{\@s{23.1} {\BY} {\DEF} UnusedS}%
 \@x{\@s{4.0}\@pfstepnum{1}{2.}\  NewSV ( S ) \.{\in} ( {\SUBSET} [
 slot \.{:} UnusedS ( S ) ,\, val \.{:} {\mathcal{V}} ] ) \.{\,\backslash\,} {\emptyset}
 \@s{2.0} {\BY}\@pfstepnum{1}{1}\  {\DEF} NewSV}%
 \@x{\@s{4.0}\@pfstepnum{1}{3.}\  \A\, t1 ,\, t2 \.{\in} NewSV ( S )
 \.{:} t1 . slot \.{=} t2 . slot \.{\implies} t1 \.{=} t2\@s{2.0}
 {\BY}\@pfstepnum{1}{1}\  {\DEF} NewSV}%
 \@x{\@s{4.0}\@pfstepnum{1}{4.}\  {\nexists}\, t1 \.{\in} MaxSV ( S ) ,\, t2
 \.{\in} ( [ slot \.{:} UnusedS ( S ) ,\, val \.{:} {\mathcal{V}} ]
 \.{\,\backslash\,} {\emptyset} ) \.{:} t1 . slot \.{=} t2 . slot}%
\@x{\@s{23.1} {\BY} {\DEF} MaxSV ,\, MaxBSV ,\, UnusedS}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{2}
 ,\,\@pfstepnum{1}{3} ,\,\@pfstepnum{1}{4}\ }%
%\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{VotedInv} asserts that if any acceptor \ensuremath{a} voted any triple \ensuremath{\langle b, s, v \rangle}, then that triple is safe.
\end{cpar}%
\end{lcom}%
 \@x{ {\LEMMA} VotedInv \.{\defeq}\@s{2.0} MsgInv \.{\land} TypeOK
 \.{\implies} \A\, a \.{\in} {\mathcal{A}} ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{81.11} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\implies} SafeAt ( b
 ,\, s ,\, v ) \.{\land} b \.{\leq} aBal [ a ]}%
 \@x{ {\BY} {\DEF} VotedForIn ,\, MsgInv ,\, Messages ,\, TypeOK ,\, MsgInv2a
 ,\, MsgInv1b ,\, MsgInv2b}%
%\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{VotedOnce} asserts that if any acceptor \ensuremath{a1} voted triple \ensuremath{\langle b, s, v1 \rangle} and acceptor \ensuremath{a2} voted triple \ensuremath{\langle b, s, v2 \rangle}, then \ensuremath{v1 = v2}.
%That is, for any given ballot and slot, only one value can be voted by any acceptor.
\end{cpar}%
\end{lcom}%
 \@x{ {\LEMMA} VotedOnce \.{\defeq} MsgInv \.{\implies} \A\, a1 ,\, a2 \.{\in}
 {\mathcal{A}} ,\, b \.{\in} {\mathcal{B}}  ,\, s \.{\in} {\mathcal{S}} ,\, v1 ,\, v2 \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{85.18} VotedForIn ( a1 ,\, b ,\, s ,\, v1 ) \.{\land} VotedForIn (
 a2 ,\, b ,\, s ,\, v2 ) \.{\implies} ( v1 \.{=} v2 )}%
 \@x{ {\BY} {\DEF} MsgInv ,\, VotedForIn ,\, MsgInv2a ,\, MsgInv1b ,\,
 MsgInv2b}%
%\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{VotedUnion} asserts that, 
%for any \ensuremath{1b} messages \ensuremath{m1} and \ensuremath{m2}, for any \ensuremath{d1} and \ensuremath{d2} in their respective \ensuremath{voted} field, if \ensuremath{d1} and \ensuremath{d2} have the same ballot and slot, then they have the same value.
in any two \ensuremath{1b} messages' \ensuremath{voted} field, triples with the same ballot and slot have the same value.
\end{cpar}%
\end{lcom}%
 \@x{ {\LEMMA} VotedUnion \.{\defeq} MsgInv \.{\land} TypeOK \.{\implies} \A\,
 m1 ,\, m2 \.{\in} msgs \.{:} m1 . type \.{=}\@w{1b} \.{\land} m2 . type
 \.{=}\@w{1b} \.{\implies}}%
 \@x{\@s{89.09} \A\, d1 \.{\in} m1 . voted ,\, d2 \.{\in} m2 . voted \.{:} (
 d1 . bal \.{=} d2 . bal \.{\land} d1 . slot \.{=} d2 . slot ) \.{\implies}}%
\@x{\@s{93.09} d1 . val \.{=} d2 . val}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} MsgInv ,\, TypeOK ,\,
 {\NEW} m1 \.{\in} msgs ,\, {\NEW} m2 \.{\in} msgs ,\, m1 . type \.{=}\@w{1b}
 ,\, m2 . type \.{=}\@w{1b} ,\,}%
 \@x{\@s{83.25} {\NEW} d1 \.{\in} m1 . voted ,\, {\NEW} d2 \.{\in} m2 . voted
 ,\, d1 . bal \.{=} d2 . bal ,\, d1 . slot \.{=} d2 . slot}%
\@x{\@s{52.31} {\PROVE} d1 . val \.{=} d2 . val \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{8.0}\@pfstepnum{1}{1.}\  VotedForIn ( m1 . from ,\, d1 . bal ,\, d1
 . slot ,\, d1 . val )\@s{2.0} {\BY} {\DEF} MsgInv ,\, MsgInv1b}%
 \@x{\@s{8.0}\@pfstepnum{1}{2.}\  VotedForIn ( m2 . from ,\, d2 . bal ,\, d2
 . slot ,\, d2 . val )\@s{2.0} {\BY} {\DEF} MsgInv ,\, MsgInv1b}%
 \@x{\@s{4.0}\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1}
 ,\,\@pfstepnum{1}{2} ,\, VotedOnce {\DEF} TypeOK ,\, Messages}%
\@pvspace{8.0pt}%

\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
The following 5 invariance lemmas 
assert that, for acceptor \ensuremath{a}, ballot \ensuremath{b}, slot \ensuremath{s}, and value \ensuremath{v}, and for all phases and preempt, if \ensuremath{VotedForIn(a, b, s, v)} holds then \ensuremath{VotedForIn(a, b, s, v)'} holds;
for all except \ensuremath{Phase2b}, the inverse also holds.
\end{cpar}%
\end{lcom}%

 \@x{ {\LEMMA} Phase1aVotedForInv \.{\defeq} TypeOK \.{\implies} \A\, p
 \.{\in} {\mathcal{P}} \.{:} Phase1a ( p ) \.{\implies} \A\, a \.{\in} {\mathcal{A}}
 ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{120.43} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\equiv} VotedForIn ( a
 ,\, b ,\, s ,\, v ) \.{'}}%
\@x{ {\BY} {\DEF} VotedForIn ,\, Send ,\, TypeOK ,\, Messages ,\, Phase1a}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} Phase1bVotedForInv \.{\defeq} TypeOK \.{\implies} \A\, a
 \.{\in} {\mathcal{A}} \.{:} Phase1b ( a ) \.{\implies} \A\, a2 \.{\in} {\mathcal{A}}
 ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{120.02} VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{\equiv} VotedForIn (
 a2 ,\, b ,\, s ,\, v ) \.{'}}%
\@x{ {\BY} {\DEF} VotedForIn ,\, Send ,\, TypeOK ,\, Messages ,\, Phase1b}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} Phase2aVotedForInv \.{\defeq} TypeOK \.{\implies} \A\, p
 \.{\in} {\mathcal{P}} \.{:} Phase2a ( p ) \.{\implies} \A\, a \.{\in} {\mathcal{A}}
 ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{120.43} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\equiv} VotedForIn ( a
 ,\, b ,\, s ,\, v ) \.{'}}%
 \@x{ {\BY} \A\, p \.{\in} {\mathcal{P}} \.{:} Phase2a ( p ) \.{\implies} \A\, m
 \.{\in} msgs \.{'} \.{\,\backslash\,} msgs \.{:} m . type \.{=}\@w{2a}
 {\DEF} VotedForIn ,\,}%
\@x{ Send ,\, TypeOK ,\, Messages ,\, Phase2a}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} Phase2bVotedForInv \.{\defeq} TypeOK \.{\implies} \A\, a
 \.{\in} {\mathcal{A}} \.{:} Phase2b ( a ) \.{\implies} \A\, a2 \.{\in} {\mathcal{A}}
 ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{120.02} VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{\implies} VotedForIn
 ( a2 ,\, b ,\, s ,\, v ) \.{'}}%
\@x{ {\BY} {\DEF} VotedForIn ,\, Send ,\, TypeOK ,\, Messages ,\, Phase2b}%
\@pvspace{8.0pt}%
 \@x{ {\LEMMA} PreemptVotedForInv \.{\defeq} TypeOK \.{\implies} \A\, p
 \.{\in} {\mathcal{P}} \.{:} Preempt ( p ) \.{\implies} \A\, a \.{\in} {\mathcal{A}}
 ,\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{119.82} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{\equiv} VotedForIn ( a
 ,\, b ,\, s ,\, v ) \.{'}}%
\@x{ {\BY} {\DEF} VotedForIn ,\, Send ,\, TypeOK ,\, Messages ,\, Preempt}%
%\@pvspace{8.0pt}%
%\@x{}\midbar\@xx{}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
Invariance lemma \ensuremath{SafeAtStable} asserts that if \ensuremath{SafeAt(b,\,s,\,v)} holds then \ensuremath{SafeAt(b,\,s,\,v)'} holds in the next state.
\end{cpar}%
\end{lcom}%
 \@x{ {\LEMMA} SafeAtStable \.{\defeq} Inv \.{\land} Next \.{\land} TypeOK
 \.{'} \.{\implies} \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in}
 {\mathcal{V}} \.{:} SafeAt ( b ,\, s ,\, v ) \.{\implies} SafeAt ( b ,\, s ,\, v
 ) \.{'}}%
 \@x{\@pfstepnum{1}{}\  {\SUFFICES} {\ASSUME} Inv ,\, Next ,\, TypeOK \.{'}
 ,\, {\NEW} b \.{\in} {\mathcal{B}} ,\, {\NEW} s \.{\in} {\mathcal{S}} ,\, {\NEW} v \.{\in}
 {\mathcal{V}} ,\, SafeAt ( b ,\, s ,\, v )}%
\@x{\@s{48.31} {\PROVE} SafeAt ( b ,\, s ,\, v ) \.{'} \@s{4.0} {\OBVIOUS}}%
\@x{\@pfstepnum{1}{}\  {\USE} {\DEF} Send ,\, Inv ,\, {\mathcal{B}}}%
 \@x{\@pfstepnum{1}{1.} {\CASE} \E\, p\@s{0.1} \.{\in} {\mathcal{P}} \.{:}
 Phase1a ( p )\@s{2.0} {\BY}\@pfstepnum{1}{1}\  {\DEF} SafeAt ,\, Phase1a ,\,
 VotedForIn ,\, WontVoteIn}%
 \@x{\@pfstepnum{1}{2.} {\CASE} \E\, a \.{\in} {\mathcal{A}}\@s{0.6} \.{:}
 Phase1b ( a )}%
 \@x{\@s{19.0} {\BY}\@pfstepnum{1}{2} ,\, QuorumAssumption {\DEF} TypeOK ,\,
 SafeAt ,\, WontVoteIn ,\, VotedForIn ,\, Phase1b}%
 \@x{\@pfstepnum{1}{3.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\, Phase2a ( p
 )\@s{2.0} {\PROVE}\@s{-4.1} SafeAt ( b ,\, s ,\, v ) \.{'}}%
 \@x{\@s{4.0}\@pfstepnum{2}{1.}\  \A\, a \.{\in} {\mathcal{A}} ,\, b2 \.{\in}
 {\mathcal{B}} ,\, s2 \.{\in} {\mathcal{S}} \.{:} WontVoteIn ( a ,\, b2 ,\, s2 ) \.{\equiv}
 WontVoteIn ( a ,\, b2 ,\, s2 ) \.{'}}%
 \@x{\@s{23.1} {\BY}\@pfstepnum{1}{3} ,\, Phase2aVotedForInv {\DEF}
 WontVoteIn ,\, Send ,\, Phase2a}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{1} ,\,
 QuorumAssumption ,\, Phase2aVotedForInv ,\,\@pfstepnum{1}{3}\  {\DEF}
 SafeAt}%
 \@x{\@pfstepnum{1}{4.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\, Phase2b ( a
 )\@s{2.0} {\PROVE} SafeAt ( b ,\, s ,\, v ) \.{'}}%
 \@x{\@s{4.0}\@pfstepnum{2}{1.}\  {\PICK} m \.{\in} msgs \.{:} Phase2b ( a )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{1}{4}\  {\DEF} Phase2b}%
 \@x{\@s{4.0}\@pfstepnum{2}{2.}\  \A\, a2 \.{\in} {\mathcal{A}} ,\, b2 \.{\in}
 {\mathcal{B}} \.{:} aBal [ a2 ] \.{>} b2 \.{\implies} aBal \.{'} [ a2 ] \.{>}
 b2\@s{2.0} {\BY}\@pfstepnum{2}{1}\  {\DEF} TypeOK}%
 \@x{\@s{4.0}\@pfstepnum{2}{3.}\  {\ASSUME} {\NEW} a2 \.{\in} {\mathcal{A}} ,\,
 {\NEW} b2 \.{\in} {\mathcal{B}} ,\, {\NEW} s2 \.{\in} {\mathcal{S}} ,\, {\NEW} v2 \.{\in}
 {\mathcal{V}} ,\, WontVoteIn ( a2 ,\, b2 ,\, s2 ) ,\,}%
 \@x{\@s{53.7} VotedForIn ( a2 ,\, b2 ,\, s2 ,\, v2 ) \.{'} ,\, {\NEW} S
 \.{\in} {\SUBSET} [ slot \.{:} {\mathcal{S}} \.{\,\backslash\,} \{ s2 \} ,\, val
 \.{:} {\mathcal{V}} ]}%
\@x{\@s{23.1} {\PROVE} {\FALSE}}%
 \@x{\@s{8.0}\@pfstepnum{3}{1.}\  \E\, m1 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} \.{\land} m1 . type \.{=}\@w{2b} \.{\land} m1
 . bal \.{=} b2 \.{\land} m1 . from \.{=} a2}%
 \@x{\@s{105.13} \.{\land} \E\, d \.{\in} m1 . propSV \.{:} d . slot \.{=} s2
 \.{\land} d . val \.{=} v2}%
\@x{\@s{27.1} {\BY}\@pfstepnum{2}{3}\  {\DEF} VotedForIn ,\, WontVoteIn}%
 \@x{\@s{8.0}\@pfstepnum{3}{2.}\  a2 \.{=} a \.{\land} m . bal \.{=}
 b2\@s{2.0} {\BY}\@pfstepnum{2}{1} ,\,\@pfstepnum{3}{1}\  {\DEF} TypeOK}%
 \@x{\@s{8.0}\@pfstepnum{3}{}\  {\QED}\@s{2.0} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{2}{3} ,\,\@pfstepnum{3}{2} ,\,\@pfstepnum{3}{1}\  {\DEF}
 Phase2b ,\, WontVoteIn ,\, TypeOK}%
 \@x{\@s{4.0}\@pfstepnum{2}{4.}\  \A\, a2 \.{\in} {\mathcal{A}} ,\, b2 \.{\in}
 {\mathcal{B}} ,\, s2 \.{\in} {\mathcal{S}} \.{:} WontVoteIn ( a2 ,\, b2 ,\, s2 )
 \.{\implies} WontVoteIn ( a2 ,\, b2 ,\, s2 ) \.{'}}%
 \@x{\@s{8.0} {\BY}\@pfstepnum{2}{2} ,\,\@pfstepnum{2}{3}\  {\DEF}
 WontVoteIn}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\QED} {\BY} Phase2bVotedForInv
 ,\,\@pfstepnum{2}{4} ,\, QuorumAssumption ,\,\@pfstepnum{1}{4}\  {\DEF}
 SafeAt}%
 \@x{\@pfstepnum{1}{5.} {\CASE} \E\, p \.{\in} {\mathcal{P}} \.{:} Preempt ( p
 )\@s{2.0} {\BY}\@pfstepnum{1}{5}\  {\DEF} SafeAt ,\, Preempt ,\, VotedForIn
 ,\, WontVoteIn}%
 \@x{\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1} ,\,\@pfstepnum{1}{2}
 ,\,\@pfstepnum{1}{3} ,\,\@pfstepnum{1}{4} ,\,\@pfstepnum{1}{5}\  {\DEF}
 Next}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Invariant} asserts the temporal formula that if \ensuremath{Spec} holds then \ensuremath{Inv} always holds. 
%Details about the proof structure and strategy can be found in Section~\ref{secProveStruct}.
\end{cpar}%
\end{lcom}%
\@x{ {\THEOREM} Invariant \.{\defeq} Spec \.{\implies} {\Box} Inv}%
\@x{\@pfstepnum{1}{}\  {\USE} {\DEF} {\mathcal{B}} ,\, {\mathcal{S}}}%
 \@x{\@pfstepnum{1}{1.}\  Init \.{\implies} Inv\@s{2.0} {\BY} FS\_EmptySet
 {\DEF} Init ,\, Inv ,\, TypeOK ,\, AccInv ,\, MsgInv ,\, VotedForIn}%
 \@x{\@pfstepnum{1}{2.}\  Inv \.{\land} [ Next ]_{ vars} \.{\implies} Inv
 \.{'}}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\SUFFICES} {\ASSUME} Inv ,\, [ Next ]_{ vars}
 {\PROVE} Inv \.{'} \@s{4.0} {\OBVIOUS}}%
\@x{\@s{4.0}\@pfstepnum{2}{}\  {\USE} {\DEF} Inv}%
\@x{\@s{4.0}\@pfstepnum{2}{1.} {\CASE} Next}%
\begin{lcom}{6.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{3}{1} proves \ensuremath{TypeOK'} for \ensuremath{Next}. 
%As described in Section~\ref{secProveStruct}, a new step is created for each action in \ensuremath{Next} and proved separately. In this case, 
Each of \@pfstepnum{4}{1-4} assumes the action of a phase and proves \ensuremath{TypeOK'} for that case.
\end{cpar}%
\end{lcom}%

\@x{\@s{4.0}\@pfstepnum{3}{1.}\  TypeOK \.{'}}%
 \@x{\@s{8.0}\@pfstepnum{4}{1.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\,
 Phase1a ( p )\@s{2.0} {\PROVE} TypeOK \.{'}}%
 \@x{\@s{27.1} {\BY}\@pfstepnum{4}{1} ,\, msgs \.{'} \.{\,\backslash\,} msgs
 \.{\subseteq} Messages ,\, FS\_AddElement {\DEF} Phase1a ,\, TypeOK ,\, Send
 ,\, Messages}%
 \@x{\@s{8.0}\@pfstepnum{4}{2.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\,
 Phase2a ( p )\@s{2.0} {\PROVE} TypeOK \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} Q \.{\in} {\mathcal{Q}} ,\, S \.{\in}
 {\SUBSET} \{ m \.{\in} msgs \.{:} ( m . type \.{=}\@w{1b} ) \.{\land} ( m .
 bal \.{=} pBal [ p ] ) \} \.{:}}%
 \@x{\@s{39.1} \.{\land} \A\, a \.{\in} Q \.{:} \E\, m \.{\in} S \.{:} m .
 from \.{=} a}%
 \@x{\@s{39.1} \.{\land} Send ( [ type \.{\mapsto}\@w{2a} ,\, from
 \.{\mapsto} p ,\, bal \.{\mapsto} pBal [ p ] ,\,}%
 \@x{\@s{51.99} propSV \.{\mapsto} PropSV ( {\UNION} \{ m . voted
 \.{:} m \.{\in} S \} ) ] )\@s{2.0} {\BY}\@pfstepnum{4}{2}\  {\DEF} Phase2a}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.}\  UnusedS ( {\UNION} \{ m . voted \.{:} m
 \.{\in} S \} ) \.{\subseteq} {\mathcal{S}}\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF}
 UnusedS ,\, TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  MaxBSV ( {\UNION} \{ m . voted \.{:} m
 \.{\in} S \} ) \.{\subseteq} [ bal \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\,
 val \.{:} {\mathcal{V}} ]}%
\@x{\@s{31.1} {\BY} {\DEF} MaxBSV ,\, TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{4.} \.{\land} NewSV ( {\UNION} \{ m .
 voted \.{:} m \.{\in} S \} ) \.{\subseteq} [ slot \.{:} {\mathcal{S}} ,\, val \.{:}
 {\mathcal{V}} ]}%
 \@x{\@s{28.44} \.{\land} MaxSV ( {\UNION} \{ m . voted \.{:} m \.{\in} S \} )
 \.{\subseteq} [ slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]\@s{2.0}
 {\BY}\@pfstepnum{5}{3} ,\,\@pfstepnum{5}{2} ,\, Misc {\DEF} MaxSV}%
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  PropSV ( {\UNION} \{ m . voted
 \.{:} m \.{\in} S \} ) \.{\subseteq} [ slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}}
 ]\@s{2.0} {\BY}\@pfstepnum{5}{4}\  {\DEF} PropSV}%
 \@x{\@s{12.0}\@pfstepnum{5}{6.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} \.{\land} m2 . type \.{=}\@w{2a} \.{\land} m2
 . from \.{=} p \.{\land} m2 . bal \.{=} pBal [ p ]}%
 \@x{\@s{109.13} \.{\land} m2 . propSV \.{=} PropSV ( {\UNION} \{ m .
 voted \.{:} m \.{\in} S \} )}%
 \@x{\@s{31.1} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{5}\  {\DEF} Send ,\,
 TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{7.}\  ( msgs \.{\subseteq} Messages )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{4}{2} ,\,\@pfstepnum{5}{6}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{5} ,\, msgs \.{'} \.{\,\backslash\,}
 msgs \.{\subseteq} Messages {\DEF} Phase2a ,\,}%
\@x{\@s{31.1} TypeOK ,\, Send ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{7}
 ,\,\@pfstepnum{4}{2} ,\, FS\_AddElement {\DEF} Phase2a ,\, TypeOK ,\, Send}%
 \@x{\@s{8.0}\@pfstepnum{4}{3.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\,
 Phase1b ( a )\@s{2.0} {\PROVE} TypeOK \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m \.{\in} msgs \.{:} Phase1b ( a )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{4}{3}\  {\DEF} Phase1b}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.} \.{\lor} msgs \.{'} \.{=} msgs \.{\cup} \{ [
 type \.{\mapsto}\@w{1b} ,\, from \.{\mapsto} a ,\, bal \.{\mapsto} m . bal
 ,\, voted \.{\mapsto} aVoted [ a ] ] \}}%
 \@x{\@s{28.44} \.{\lor} msgs \.{'} \.{=} msgs \.{\cup} \{ [ type
 \.{\mapsto}\@w{preempt} ,\, to \.{\mapsto} m . from ,\, bal \.{\mapsto} aBal
 [ a ] ] \}\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} \.{\lor} m2 . type \.{=}\@w{1b} \.{\land} m2 .
 from \.{=} a \.{\land} m2 . bal \.{=} m . bal \.{\land} m2 . voted \.{=}
 aVoted [ a ]}%
 \@x{\@s{109.13} \.{\lor} m2 . type \.{=}\@w{preempt} \.{\land} m2 . to \.{=}
 m . from \.{\land} m2 . bal \.{=} aBal [ a ]}%
\@x{\@s{31.1} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send}%
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  ( msgs \.{\subseteq} Messages )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{3}\  {\DEF} TypeOK
 ,\, Messages ,\, Send}%
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  IsFiniteSet ( msgs ) \.{'}\@s{2.0}
 {\BY}\@pfstepnum{5}{2} ,\, FS\_AddElement {\DEF} TypeOK}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{4}
 ,\,\@pfstepnum{5}{5} ,\,\@pfstepnum{4}{3}\  {\DEF} Phase1b ,\, TypeOK}%
 \@x{\@s{8.0}\@pfstepnum{4}{4.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\,
 Phase2b ( a )\@s{2.0} {\PROVE} TypeOK \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m \.{\in} msgs \.{:} Phase2b ( a )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{4}{4}\  {\DEF} Phase2b}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.} \.{\lor} msgs \.{'} \.{=} msgs \.{\cup} \{ [
 type \.{\mapsto}\@w{2b} ,\, bal \.{\mapsto} m . bal ,\, from \.{\mapsto} a
 ,\, propSV \.{\mapsto} m . propSV ] \}}%
 \@x{\@s{28.44} \.{\lor} msgs \.{'} \.{=} msgs \.{\cup} \{ [ type
 \.{\mapsto}\@w{preempt} ,\, to \.{\mapsto} m . from ,\, bal \.{\mapsto} aBal
 [ a ] ] \}\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  IsFiniteSet ( msgs ) \.{'}\@s{2.0}
 {\BY}\@pfstepnum{5}{2} ,\, FS\_AddElement {\DEF} TypeOK}%
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} \.{\lor} m2 . type \.{=}\@w{2b} \.{\land} m2 .
 from \.{=} a \.{\land} m2 . bal \.{=} m . bal \.{\land} m2 . propSV \.{=} m
 . propSV}%
 \@x{\@s{109.13} \.{\lor} m2 . type \.{=}\@w{preempt} \.{\land} m2 . to \.{=}
 m . from \.{\land} m2 . bal \.{=} aBal [ a ]}%
\@x{\@s{31.1} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send}%
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  ( msgs \.{\subseteq} Messages )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{4}\  {\DEF} TypeOK
 ,\, Send ,\, Messages}%
\@x{\@s{12.0}\@pfstepnum{5}{6.} \.{\lor} aVoted \.{=} aVoted \.{'}}%
 \@x{\@s{28.44} \.{\lor} \.{\land} {\DOMAIN} aVoted \.{=} {\DOMAIN} aVoted
 \.{'}}%
 \@x{\@s{37.33} \.{\land} aVoted \.{'} [ a ] \.{=} \{ d \.{\in} aVoted [ a ]
 \.{:} {\nexists}\, d2 \.{\in} m . propSV \.{:} d . slot \.{=} d2 . slot \}
 \.{\cup}}%
 \@x{\@s{94.38} \{ [ bal \.{\mapsto} m . bal ,\, slot \.{\mapsto} d . slot
 ,\, val \.{\mapsto} d . val ] \.{:} d \.{\in} m . propSV \}}%
 \@x{\@s{37.33} \.{\land} \A\, a2 \.{\in} {\mathcal{A}} \.{\,\backslash\,} \{ a \}
 \.{:} aVoted [ a2 ] \.{=} aVoted \.{'} [ a2 ]\@s{2.0}
 {\BY}\@pfstepnum{5}{1}\  {\DEF} TypeOK}%
 \@x{\@s{12.0}\@pfstepnum{5}{7.}\  ( aVoted \.{\in} [ {\mathcal{A}}
 \.{\rightarrow} {\SUBSET} [ bal \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val
 \.{:} {\mathcal{V}} ] ] ) \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{6}
 ,\,}%
 \@x{\@s{31.1} \{ [ bal \.{\mapsto} m . bal ,\, slot \.{\mapsto} d . slot ,\,
 val \.{\mapsto} d . val ] \.{:} d \.{\in} m . propSV \} \.{\subseteq} [ bal
 \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\,}%
 \@x{\@s{31.1} \{ d \.{\in} aVoted [ a ] \.{:} {\nexists}\, d2 \.{\in} m .
 propSV \.{:} d . slot \.{=} d2 . slot \} \.{\subseteq} [ bal \.{:} {\mathcal{B}}
 ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] ,\,}%
 \@x{\@s{31.1} aVoted \.{'} [ a ] \.{\subseteq} [ bal \.{:} {\mathcal{B}} ,\, slot
 \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ] {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{5}
 ,\,\@pfstepnum{5}{7} ,\,\@pfstepnum{4}{4} ,\,\@pfstepnum{5}{3}\  {\DEF}
 Phase2b ,\, TypeOK}%
\begin{lcom}{10.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{4}{5} proves \ensuremath{TypeOK'} for \ensuremath{Preempt}. This is the new part of the remedial proof described in Section~\ref{secMadeupProof}.
\end{cpar}%
\end{lcom}%

 \@x{\@s{8.0}\@pfstepnum{4}{5.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\,
 Preempt ( p )\@s{2.0} {\PROVE} TypeOK \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\DEFINE} S \.{\defeq} \{ m1 \.{\in} msgs
 \.{:} m1 . type \.{=}\@w{1a} \}\@s{2.0} T \.{\defeq} \{ s . bal \.{:} s
 \.{\in} S \}\@s{2.0} f \.{\defeq} [ s \.{\in} S \.{\mapsto} s . bal ]}%
\@x{\@s{12.0}\@pfstepnum{5}{}\  {\HIDE} {\DEF} S ,\, T ,\, f}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m \.{\in} msgs \.{:} Preempt ( p )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{4}{5}\  {\DEF} Preempt}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.}\  T \.{\subseteq} {\mathcal{B}}\@s{2.0} {\BY}
 {\DEF} T ,\, S ,\, TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  \E\, b \.{\in} {\mathcal{B}} \.{:} b \.{>} m .
 bal \.{\land} b \.{\notin} T}%
 \@x{\@s{31.1} {\BY}\@pfstepnum{5}{2} ,\, MaxInSet ,\, Max ( T \.{\cup} \{ m
 . bal \} ) \.{+} 1 \.{>} m . bal ,\,\@pfstepnum{5}{1}\  {\DEF} Max ,\,
 TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  NewBal ( m . bal ) \.{\in}
 {\mathcal{B}}\@s{2.0} {\BY}\@pfstepnum{5}{3}\  {\DEF} NewBal ,\, TypeOK ,\,
 Messages ,\, T ,\, S}%
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  ( pBal \.{\in} [ {\mathcal{P}} \.{\rightarrow}
 {\mathcal{B}} ] ) \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{4}\ 
 {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{4}{5}
 ,\,\@pfstepnum{5}{5}\  {\DEF} Preempt ,\, TypeOK}%
 \@x{\@s{8.0}\@pfstepnum{4}{}\  {\QED} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{4}{1} ,\,\@pfstepnum{4}{2} ,\,\@pfstepnum{4}{3}
 ,\,\@pfstepnum{4}{4} ,\,\@pfstepnum{4}{5}\  {\DEF} Next}%
\@pvspace{8.0pt}%
\begin{lcom}{6.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{3}{2} proves \ensuremath{AccInv'} for \ensuremath{Next}.  
%It uses the same strategy as for proving \ensuremath{TypeOK'} in \@pfstepnum{3}{1}.
Each of \@pfstepnum{4}{1-4} assumes the action of a phase and proves \ensuremath{AccInv'} for that case.\\
Only \ensuremath{Phase2b} is challenging because only it updates acceptor variables.
\end{cpar}\end{lcom}
\@x{\@s{4.0}\@pfstepnum{3}{2.}\  AccInv \.{'}}%
 \@x{\@s{8.0}\@pfstepnum{4}{1.} {\CASE} \E\, p \.{\in} {\mathcal{P}} \.{:}
 Phase1a ( p )\@s{2.0} {\BY}\@pfstepnum{4}{1} ,\,\@pfstepnum{3}{1} ,\,
 Phase1aVotedForInv {\DEF} AccInv ,\, TypeOK ,\, Phase1a ,\, Send}%
 \@x{\@s{8.0}\@pfstepnum{4}{2.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\,
 Phase2a ( p )\@s{2.0} {\PROVE} AccInv \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  \A\, a \.{\in} {\mathcal{A}} ,\, b \.{\in}
 {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} VotedForIn ( a ,\, b
 ,\, s ,\, v ) \.{\equiv} VotedForIn ( a ,\, b ,\, s ,\, v ) \.{'}}%
\@x{\@s{31.1} {\BY}\@pfstepnum{4}{2} ,\, Phase2aVotedForInv}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{3}{1}
 ,\,\@pfstepnum{4}{2} ,\,\@pfstepnum{5}{1}\  {\DEF} AccInv ,\, TypeOK ,\,
 Phase2a ,\, Send ,\, Messages}%
 \@x{\@s{8.0}\@pfstepnum{4}{3.} {\CASE} \E\, a \.{\in} {\mathcal{A}} \.{:}
 Phase1b ( a )\@s{2.0} {\BY}\@pfstepnum{4}{3} ,\,\@pfstepnum{3}{1} ,\,
 Phase1bVotedForInv {\DEF} AccInv ,\, TypeOK ,\, Phase1b ,\, Send}%
%\begin{lcom}{10.5}%
%\begin{cpar}{0}{F}{F}{0}{0}{}%
% To prove \ensuremath{AccInv'}, only \ensuremath{Phase2b} is challenging because only it updates acceptor variables.
%\end{cpar}\end{lcom}
 \@x{\@s{8.0}\@pfstepnum{4}{4.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\,
 Phase2b ( a )\@s{2.0} {\PROVE} AccInv \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\SUFFICES} {\ASSUME} {\NEW} a2 \.{\in}
 {\mathcal{A}} \.{'}}%
 \@x{\@s{60.31} {\PROVE} ( \.{\land} aBal [ a2 ] \.{=} \.{-} 1
 \.{\implies} aVoted [ a2 ] \.{=} {\emptyset}}%
 \@x{\@s{93.38} \.{\land} \A\, r \.{\in} aVoted [ a2 ] \.{:} VotedForIn ( a2
 ,\, r . bal ,\, r . slot ,\, r . val ) \.{\land} r . bal \.{\leq} aBal [ a2
 ]}%
 \@x{\@s{93.38} \.{\land} \A\, b\@s{0.05} \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}}
 ,\, v \.{\in} {\mathcal{V}} \.{:}}%
 \@x{\@s{106.27} \.{\land} VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{\implies}
 \E\, r \.{\in} aVoted [ a2 ] \.{:} r . bal \.{\geq} b \.{\land} r . slot
 \.{=} s}%
 \@x{\@s{106.27} \.{\land} b \.{>} MaxBalInSlot ( aVoted [ a2 ] ,\, s )
 \.{\implies} {\lnot} VotedForIn ( a2 ,\, b ,\, s ,\, v ) ) \.{'}}%
\@x{\@s{60.31} {\BY} {\DEF} AccInv}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m \.{\in} msgs \.{:} Phase2b ( a )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{4}{4}\  {\DEF} Phase2b}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{5}{2} assumes that \ensuremath{a} received a \textsf{2a} message with a ballot lower than the highest it has seen, %annie: why write with negation in proof sc - i don't think its necessary but what I've written in <5>2 is the negation of <5>3. I remember that the solvers have trouble figuring out negations on quantified expressions but may be not in this one because there is no quantification.
thus triggering preemption. This case is simple as acceptor variables are unchanged.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{2.} {\CASE} ( a2 \.{=} a \.{\land} {\lnot} ( m .
 bal \.{\geq} aBal [ a ] ) ) \.{\lor} a2 \.{\neq} a}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in} {\mathcal{S}}
 ,\, v \.{\in} {\mathcal{V}} \.{:} VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{\equiv}
 VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{'}}%
 \@x{\@s{35.1} {\BY}\@pfstepnum{3}{1} ,\,\@pfstepnum{5}{1}
 ,\,\@pfstepnum{5}{2}\  {\DEF} Phase2b ,\, TypeOK ,\, {\mathcal{B}} ,\, Messages
 ,\, VotedForIn ,\, Send}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{2} ,\,\@pfstepnum{4}{4}
 ,\,\@pfstepnum{3}{1}\  {\DEF} Phase2b ,\, Send ,\, AccInv ,\, TypeOK ,\,
 Messages}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{5}{3} assumes that \ensuremath{a} received a \textsf{2a} message with a ballot higher than or equal to the highest it has seen. Thus, it responds with a \textsf{2b} message and updates its variables as specified. Each of \@pfstepnum{6}{1-4} proves a conjunct of \ensuremath{AccInv}.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{3.} {\CASE} a2 \.{=} a \.{\land} ( m . bal
 \.{\geq} aBal [ a ] )}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  ( aBal [ a2 ] \.{=} \.{-} 1 \.{\implies}
 aVoted [ a2 ] \.{=} {\emptyset} ) \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{3}
 ,\,\@pfstepnum{4}{4} ,\,\@pfstepnum{3}{1}\  {\DEF} AccInv ,\, Phase2b ,\,
 Send ,\,}%
\@x{\@s{35.1} TypeOK ,\, Messages}%
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  ( \A\, r \.{\in} aVoted [ a2 ] \.{:}
 VotedForIn ( a2 ,\, r . bal ,\, r . slot ,\, r . val ) \.{\land} r . bal
 \.{\leq} aBal [ a2 ] ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\SUFFICES} {\ASSUME} {\NEW} r \.{\in} (
 aVoted [ a2 ] ) \.{'}}%
 \@x{\@s{68.31} {\PROVE} ( VotedForIn ( a2 ,\, r . bal ,\, r . slot
 ,\, r . val ) \.{\land} r . bal \.{\leq} aBal [ a2 ] ) \.{'} \@s{4.0} {\OBVIOUS}}%
\begin{lcom}{22.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{7}{1} uses two cases. \@pfstepnum{8}{1} is for \ensuremath{r \in aVoted[a2]} and uses invariance lemma for  \ensuremath{Phase2b}. \@pfstepnum{8}{2} is for the increment \ensuremath{r \in aVoted'[a2] \setminus aVoted[a2]} and uses definition of \ensuremath{Phase2b}.
\end{cpar}\end{lcom}
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  VotedForIn ( a2 ,\, r . bal ,\, r . slot
 ,\, r . val ) \.{'}}%
\@x{\@s{24.0}\@pfstepnum{8}{1.} {\CASE} r \.{\in} aVoted [ a2 ]}%
 \@x{\@s{28.0}\@pfstepnum{9}{1.}\  VotedForIn ( a2 ,\, r . bal ,\, r . slot
 ,\, r . val )\@s{2.0} {\BY}\@pfstepnum{5}{3} ,\,\@pfstepnum{4}{4}
 ,\,\@pfstepnum{8}{1}\  {\DEF} AccInv}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{9}{1} ,\,
 Phase2bVotedForInv ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{4}{4}\  {\DEF} TypeOK
 ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.} {\CASE} r \.{\in} aVoted \.{'} [ a2 ]
 \.{\,\backslash\,} aVoted [ a2 ]}%
 \@x{\@s{28.0}\@pfstepnum{9}{1.}\  \E\, m2 \.{\in} msgs \.{'} \.{:} m2 . type
 \.{=}\@w{2b} \.{\land} m2 . from \.{=} a2 \.{\land} m2 . bal \.{=} m . bal
 \.{\land} m2 . propSV \.{=} m . propSV}%
 \@x{\@s{47.1} {\BY}\@pfstepnum{3}{1} ,\,\@pfstepnum{8}{2}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{3}\  {\DEF} Send}%
 \@x{\@s{28.0}\@pfstepnum{9}{2.}\  r . bal \.{=} m . bal \.{\land} \E\, d
 \.{\in} m . propSV \.{:} r . slot \.{=} d . slot \.{\land} r . val \.{=} d
 . val\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{3}
 ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{8}{2}\ }%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{9}{1}
 ,\,\@pfstepnum{9}{2}\  {\DEF} Send ,\, TypeOK ,\, Messages ,\, VotedForIn}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{1}
 ,\,\@pfstepnum{8}{2}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{2.}\  ( r . bal \.{\leq} aBal [ a2 ] )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{3}
 ,\,\@pfstepnum{3}{1} ,\, aBal [ a ] \.{\leq} aBal \.{'} [ a ] ,\, r \.{\in}
 aVoted [ a ] \.{\implies} r . bal \.{\leq} aBal \.{'} [ a ] ,\,}%
 \@x{\@s{39.1} aVoted \.{'} [ a ] \.{=} \{ d \.{\in} aVoted [ a ] \.{:}
 {\nexists}\, d2 \.{\in} m . propSV \.{:} d . slot \.{=} d2 . slot \}
 \.{\cup}}%
 \@x{\@s{87.27} \{ [ bal \.{\mapsto} m . bal ,\, slot \.{\mapsto} d . slot
 ,\, val \.{\mapsto} d . val ] \.{:} d \.{\in} m . propSV \} ,\,}%
 \@x{\@s{39.1} r \.{\in} aVoted \.{'} [ a2 ] \.{\,\backslash\,} aVoted [ a2 ]
 \.{\implies} r . bal \.{=} m . bal}%
\@x{\@s{30.0} {\DEF} AccInv ,\, Send ,\, TypeOK ,\, Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}
 ,\,\@pfstepnum{7}{2}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{3.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} VotedForIn ( a2 ,\, b ,\, s ,\, v )
 \.{\implies} \E\, r \.{\in} aVoted [ a2 ] \.{:} r . bal \.{\geq} b \.{\land}
 r . slot \.{=} s ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\SUFFICES} {\ASSUME} {\NEW} b \.{\in}
 {\mathcal{B}} \.{'} ,\, {\NEW} s \.{\in} {\mathcal{S}} \.{'} ,\, {\NEW} v \.{\in} {\mathcal{V}}
 \.{'} ,\, VotedForIn ( a2 ,\, b ,\, s ,\, v ) \.{'}}%
 \@x{\@s{68.31} {\PROVE} ( \E\, r \.{\in} aVoted [ a2 ] \.{:} r . bal
 \.{\geq} b \.{\land} r . slot \.{=} s ) \.{'} \@s{4.0} {\OBVIOUS}}%
\@x{\@s{20.0}\@pfstepnum{7}{1.} {\CASE} VotedForIn ( a2 ,\, b ,\, s ,\, v )}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  {\PICK} r \.{\in} aVoted [ a2 ] \.{:} r .
 bal \.{\geq} b \.{\land} r . slot \.{=} s\@s{2.0} {\BY}\@pfstepnum{7}{1}\ 
 {\DEF} AccInv ,\, TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  m . bal \.{\geq} b\@s{2.0}
 {\BY}\@pfstepnum{8}{1} ,\,\@pfstepnum{5}{3}\  {\DEF} TypeOK ,\, Messages ,\,
 AccInv}%
 \@x{\@s{24.0}\@pfstepnum{8}{3.} {\CASE} \E\, d \.{\in} m . propSV \.{:} d .
 slot \.{=} s}%
 \@x{\@s{28.0}\@pfstepnum{9}{1.}\  \E\, r2 \.{\in} aVoted \.{'} [ a ] \.{:} r2
 . bal \.{=} m . bal \.{\land} r2 . slot \.{=} s {\BY}\@pfstepnum{5}{1}
 ,\,\@pfstepnum{5}{3} ,\,}%
 \@x{\@s{47.1} aVoted \.{'} [ a ] \.{=} \{ d \.{\in} aVoted [ a ] \.{:}
 {\nexists}\, d2 \.{\in} m . propSV \.{:} d . slot \.{=} d2 . slot \}
 \.{\cup}}%
 \@x{\@s{47.1} \{ [ bal \.{\mapsto} m . bal ,\, slot \.{\mapsto} d . slot ,\,
 val \.{\mapsto} d . val ] \.{:} d \.{\in} m . propSV \}
 ,\,\@pfstepnum{8}{3}\  {\DEF} TypeOK}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{9}{1}
 ,\,\@pfstepnum{5}{3} ,\,\@pfstepnum{8}{2}\ }%
 \@x{\@s{24.0}\@pfstepnum{8}{4.} {\CASE} {\nexists}\, d \.{\in} m . propSV
 \.{:} d . slot \.{=} s\@s{2.0} {\BY}\@pfstepnum{8}{4} ,\,\@pfstepnum{8}{1}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{3} ,\, r \.{\in} aVoted \.{'} [ a2 ]}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{3}
 ,\,\@pfstepnum{8}{4}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{2.} {\CASE} {\lnot} VotedForIn ( a2 ,\, b ,\, s
 ,\, v )}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  \E\, d \.{\in} m . propSV \.{:} d . slot
 \.{=} s\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{7}{2}\  {\DEF} Send
 ,\, TypeOK ,\, Messages ,\, VotedForIn}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  \E\, r\@s{0.68} \.{\in} aVoted \.{'} [ a2 ]
 \.{:} r . bal \.{=} m . bal \.{\land} r . slot \.{=} s\@s{2.0}
 {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{8}{1} ,\,\@pfstepnum{2}{1}
 ,\,\@pfstepnum{5}{3}\  {\DEF} Send ,\, TypeOK ,\,}%
\@x{\@s{43.1} Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{3.}\  b \.{=} m . bal\@s{2.0}
 {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{7}{2} ,\,\@pfstepnum{5}{3}\  {\DEF}
 VotedForIn ,\, Send}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{2}
 ,\,\@pfstepnum{8}{3}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}
 ,\,\@pfstepnum{7}{2}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{4.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b \.{>} MaxBalInSlot ( aVoted [ a2 ] ,\,
 s ) \.{\implies} {\lnot} VotedForIn ( a2 ,\, b ,\, s ,\, v ) ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\SUFFICES} {\ASSUME} {\NEW} b \.{\in}
 {\mathcal{B}} \.{'} ,\, {\NEW} s \.{\in} {\mathcal{S}} \.{'} ,\, {\NEW} v \.{\in} {\mathcal{V}}
 \.{'} ,\, ( VotedForIn ( a2 ,\, b ,\, s ,\, v ) ) \.{'} ,\,}%
\@x{\@s{98.91} ( b \.{>} MaxBalInSlot ( aVoted [ a2 ] ,\, s ) ) \.{'}}%
\@x{\@s{68.31} {\PROVE} {\FALSE} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  {\nexists}\, d \.{\in} aVoted \.{'} [ a2 ]
 \.{:} d . slot \.{=} s \.{\land} d . bal \.{>} MaxBalInSlot ( aVoted [ a2
 ] ,\, s ) \.{'}}%
\@x{\@s{39.1} {\BY} MaxBinSNoMore ,\,\@pfstepnum{3}{1}\  {\DEF} TypeOK}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}
 ,\,\@pfstepnum{6}{3} ,\, \E\, r \.{\in} aVoted \.{'} [ a2 ] \.{:} r . bal
 \.{\geq} b \.{\land} r . slot \.{=} s ,\, MaxBinSType ,\,\@pfstepnum{3}{1}\ 
 {\DEF} Send ,\,}%
\@x{\@s{32.89} TypeOK ,\, Messages}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2} ,\,\@pfstepnum{6}{3} ,\,\@pfstepnum{6}{4}\ }%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{2}
 ,\,\@pfstepnum{5}{3}\ }%
 \@x{\@s{8.0}\@pfstepnum{4}{5.} {\CASE} \E\, p \.{\in} {\mathcal{P}} \.{:}
 Preempt ( p )}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  \A\, a \.{\in} {\mathcal{A}} ,\, s \.{\in}
 {\mathcal{S}} \.{:} MaxBalInSlot ( aVoted [ a ] ,\, s ) \.{=} MaxBalInSlot (
 aVoted [ a ] ,\, s ) \.{'}}%
 \@x{\@s{31.1} {\BY}\@pfstepnum{3}{1} ,\,\@pfstepnum{4}{5}\  {\DEF} Preempt
 ,\, MaxBalInSlot}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{4}{5}
 ,\,\@pfstepnum{3}{1} ,\, PreemptVotedForInv ,\,\@pfstepnum{5}{1}\  {\DEF}
 AccInv ,\, TypeOK ,\, Preempt ,\, Send}%
 \@x{\@s{8.0}\@pfstepnum{4}{} . {\QED} {\BY}\@pfstepnum{4}{1}
 ,\,\@pfstepnum{4}{2} ,\,\@pfstepnum{4}{3} ,\,\@pfstepnum{4}{4}
 ,\,\@pfstepnum{4}{5} ,\,\@pfstepnum{2}{1}\  {\DEF} Next}%
\@pvspace{8.0pt}%
\begin{lcom}{6.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{3}{3} proves \ensuremath{MsgInv'} for \ensuremath{Next}. 
 %It uses the same strategy as for proving \ensuremath{TypeOK'} in \@pfstepnum{3}{1}.
 Each of \@pfstepnum{4}{1-4} assumes the action of a phase and proves \ensuremath{MsgInv'} for that case.
\end{cpar}\end{lcom}
\@x{\@s{4.0}\@pfstepnum{3}{3.}\  MsgInv \.{'}}%
 \@x{\@s{8.0}\@pfstepnum{4}{1.} {\CASE} \E\, p \.{\in} {\mathcal{P}} \.{:}
 Phase1a ( p )\@s{2.0} {\BY}\@pfstepnum{4}{1} ,\, Phase1aVotedForInv
 ,\,\@pfstepnum{3}{1} ,\, SafeAtStable ,\,\@pfstepnum{2}{1}\ }%
 \@x{\@s{18.0} {\DEF} Phase1a ,\, MsgInv ,\, Send ,\, TypeOK ,\, Messages ,\,
 MsgInv1b ,\, MsgInv2a ,\, MsgInv2b}%
\begin{lcom}{10.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{4}{2} proves \ensuremath{MsgInv'} for \ensuremath{Phase1b}. \@pfstepnum{5}{13,14} conclude the proof while \@pfstepnum{5}{1-12} prove intermediate facts. Each of \@pfstepnum{5}{2,4,12} proves a conjunct of \ensuremath{MsgInv1b} for the increment \ensuremath{m1}---the new \ensuremath{1b} message sent in \ensuremath{Phase1b(a)}.
\end{cpar}\end{lcom}
 \@x{\@s{8.0}\@pfstepnum{4}{2.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\,
 Phase1b ( a )\@s{2.0} {\PROVE} MsgInv \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\DEFINE} m1 \.{\defeq} [ type
 \.{\mapsto}\@w{1b} ,\, from \.{\mapsto} a ,\, bal \.{\mapsto} m . bal ,\,
 voted \.{\mapsto} aVoted [ a ] ]}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m \.{\in} msgs \.{:} Phase1b ( a )
 {\bang} ( m )\@s{2.0} {\BY}\@pfstepnum{4}{2}\  {\DEF} Phase1b}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.}\  ( m1 . bal \.{\leq} aBal [ m1 . from ] )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{1}\  {\DEF} Phase1b
 ,\, Send ,\, TypeOK ,\, MsgInv ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  m1 . voted \.{=} aVoted [ m1 . from
 ]\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{1}\  {\DEF} Phase1b ,\,
 Send ,\, TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  ( \A\, r \.{\in} m1 . voted \.{:}
 VotedForIn ( m1 . from ,\, r . bal ,\, r . slot ,\, r . val ) ) \.{'}}%
 \@x{\@s{31.1} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{4}{2} ,\,
 Phase1bVotedForInv ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{5}{3}\  {\DEF} TypeOK
 ,\, Messages ,\, AccInv}%
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b \.{>} MaxBalInSlot ( m1 . voted ,\, s
 ) \.{\implies} {\lnot} VotedForIn ( m1 . from ,\, b ,\, s ,\, v ) ) \.{'}}%
 \@x{\@s{31.1} {\BY} Phase1bVotedForInv ,\,\@pfstepnum{4}{2}
 ,\,\@pfstepnum{5}{3} ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{2}
 ,\,\@pfstepnum{3}{1}\  {\DEF} AccInv ,\, MsgInv ,\, Send ,\, TypeOK ,\,
 Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{6.}\  \A\, s \.{\in} {\mathcal{S}} \.{:} MaxBalInSlot
 ( m1 . voted ,\, s ) \.{\in} {\mathcal{B}} \.{\cup} \{ \.{-} 1 \}\@s{2.0}
 {\BY}\@pfstepnum{3}{1} ,\, MaxBinSType {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{7.}\  \A\, s \.{\in} {\mathcal{S}} \.{:} \.{\land} MaxBalInSlot
 ( m1 . voted ,\, s ) \.{+} 1 \.{\in} {\mathcal{B}}}%
 \@x{\@s{63.0} \.{\land} MaxBalInSlot
 ( m1 . voted ,\, s ) \.{+} 1 \.{>} MaxBalInSlot ( m1 . voted ,\, s )}%
\@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} {\NEW} s \.{\in} {\mathcal{S}}}%
 \@x{\@s{64.31} {\PROVE} \.{\land} MaxBalInSlot
 ( m1 . voted ,\, s ) \.{+} 1 \.{>} MaxBalInSlot ( m1 . voted ,\, s )}%
 \@x{\@s{95.0} \.{\land} MaxBalInSlot ( m1 . voted ,\, s ) \.{+} 1
 \.{\in} {\mathcal{B}}\@s{4.0} {\OBVIOUS}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.} {\CASE} MaxBalInSlot ( m1 . voted ,\, s )
 \.{=} \.{-} 1\@s{2.0} {\BY}\@pfstepnum{6}{1}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{2.} {\CASE} MaxBalInSlot ( m1 . voted ,\, s )
 \.{\in} {\mathcal{B}}\@s{2.0} {\BY} \A\, x \.{\in} {\mathcal{B}} \.{:} x \.{+} 1 \.{>} x
 ,\,\@pfstepnum{6}{2}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2} ,\,\@pfstepnum{5}{6}\ }%
 \@x{\@s{12.0}\@pfstepnum{5}{9.}\  m1 . bal \.{\in} {\mathcal{B}}\@s{2.0}
 {\BY}\@pfstepnum{3}{1}\  {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{12.0}\@pfstepnum{5}{10.}\  \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} \.{:} b \.{\in} MaxBalInSlot ( m1 . voted ,\, s ) \.{+} 1
 \.{\dotdot} m1 . bal \.{-} 1 \.{\implies} b \.{>} MaxBalInSlot ( m1 . voted ,\, s )}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} {\NEW} b \.{\in}
 {\mathcal{B}} ,\, {\NEW} s \.{\in} {\mathcal{S}} ,\, b \.{\in} MaxBalInSlot ( m1 .
 voted ,\, s ) \.{+} 1 \.{\dotdot} m1 . bal \.{-} 1}%
\@x{\@s{64.31} {\PROVE} b \.{>} MaxBalInSlot ( m1 . voted ,\, s ) \@s{4.0} {\OBVIOUS}}%
\@x{\@s{16.0}\@pfstepnum{6}{}\  {\HIDE} {\DEF} m1}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\DEFINE} x \.{\defeq} MaxBalInSlot ( m1 .
 voted ,\, s )\@s{2.0} y \.{\defeq} m1 . bal \.{-} 1}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  x \.{\in} {\mathcal{B}} \.{\cup} \{ \.{-} 1
 \}\@s{2.0} {\BY}\@pfstepnum{5}{6}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  y\@s{0.08} \.{\in} {\mathcal{B}} \.{\cup} \{
 \.{-} 1 \}\@s{2.0} {\BY}\@pfstepnum{5}{9}\ }%
\@x{\@s{16.0}\@pfstepnum{6}{}\  {\HIDE} {\DEF} x ,\, y}%
\@x{\@s{16.0}\@pfstepnum{6}{3.} {\CASE} x \.{+} 1 \.{>} y}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  \A\, e \.{\in} {\mathcal{B}} \.{:} e \.{\notin} x
 \.{+} 1 \.{\dotdot} y\@s{2.0} {\BY}\@pfstepnum{6}{3} ,\,\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{6}{3}
 ,\,\@pfstepnum{7}{1}\  {\DEF} x ,\, y}%
 \@x{\@s{16.0}\@pfstepnum{6}{4.} {\CASE} x \.{+} 1 \.{=} y\@s{2.0}
 {\BY}\@pfstepnum{6}{4} ,\,\@pfstepnum{5}{7}
 ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{5}{9}\  {\DEF} x ,\, y}%
\@x{\@s{16.0}\@pfstepnum{6}{5.} {\CASE} x \.{+} 1 \.{<} y}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  \A\, e \.{\in} {\mathcal{B}} \.{:} e \.{\in} x
 \.{+} 1 \.{\dotdot} y \.{\implies} e \.{>} x\@s{2.0} {\BY}\@pfstepnum{6}{5}
 ,\,\@pfstepnum{6}{1} ,\,\@pfstepnum{6}{2}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{2.}\  b \.{\in} x \.{+} 1 \.{\dotdot} y\@s{2.0}
 {\BY} {\DEF} x ,\, y}%
 \@x{\@s{20.0}\@pfstepnum{7}{3.}\  b \.{>} x\@s{2.0} {\BY}\@pfstepnum{7}{2}
 ,\,\@pfstepnum{7}{1}\ }%
\@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{3}\  {\DEF} x}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{3}
 ,\,\@pfstepnum{6}{4} ,\,\@pfstepnum{6}{5} ,\,\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\ }%
 \@x{\@s{12.0}\@pfstepnum{5}{11.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} \.{:} b \.{\in} MaxBalInSlot ( m1 . voted ,\, s ) \.{+} 1
 \.{\dotdot} m1 . bal \.{-} 1 \.{\implies}}%
 \@x{\@s{40.22} b \.{>} MaxBalInSlot ( m1 . voted ,\, s ) ) \.{'}\@s{2.0}
 {\BY}\@pfstepnum{5}{10} ,\,\@pfstepnum{5}{1}\ }%
 \@x{\@s{12.0}\@pfstepnum{5}{12.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b \.{\in} MaxBalInSlot ( m1 . voted ,\,
 s ) \.{+} 1 \.{\dotdot} m1 . bal \.{-} 1 \.{\implies}}%
\@x{\@s{40.22} {\lnot} VotedForIn ( m1 . from ,\, b ,\, s ,\, v ) ) \.{'}}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} {\NEW} b \.{\in}
 {\mathcal{B}} \.{'} ,\, {\NEW} s \.{\in} {\mathcal{S}} \.{'} ,\, {\NEW} v \.{\in} {\mathcal{V}}
 \.{'}}%
 \@x{\@s{64.31} {\PROVE} ( b \.{\in} MaxBalInSlot ( m1 . voted ,\,
 s ) \.{+} 1 \.{\dotdot} m1 . bal \.{-} 1 \.{\implies}}%
\@x{\@s{102.93} {\lnot} VotedForIn ( m1 . from ,\, b ,\, s ,\, v ) ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.} {\CASE} {\nexists}\, x \.{\in} {\mathcal{B}} \.{:}
 x \.{\in} ( MaxBalInSlot ( m1 . voted ,\, s ) \.{+} 1 \.{\dotdot} m1 .
 bal \.{-} 1 ) \.{'}\@s{2.0} {\BY}\@pfstepnum{6}{1}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{2.} {\CASE} \E\, x \.{\in} {\mathcal{B}} \.{:} x
 \.{\in} ( MaxBalInSlot ( m1 . voted ,\, s ) \.{+} 1 \.{\dotdot} m1 . bal
 \.{-} 1 ) \.{'}\@s{2.0} {\BY}\@pfstepnum{6}{2} ,\,\@pfstepnum{5}{5}
 ,\,\@pfstepnum{5}{11}\ }%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\ }%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\@pfstepnum{5}{13} is for \textsf{1a} message $m$ having a higher ballot than the highest seen, thus generating a \textsf{1b} message. %annie: what about 2b? sc - this is Phase1b, so no new 2b or 2a messages, right?
\end{cpar}\end{lcom}
\@x{\@s{12.0}\@pfstepnum{5}{13.} {\CASE} m . bal \.{>} aBal [ a ]}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} {\NEW} m2 \.{\in} msgs
 \.{'}}%
 \@x{\@s{64.31} {\PROVE} ( \.{\land} ( m2 . type \.{=}\@w{1b} )
 \.{\implies} MsgInv1b ( m2 ) \.{\land} ( m2 . type\@s{1.1} \.{=}\@w{2a} )\@s{0.29}
 \.{\implies} MsgInv2a ( m2 )}%
 \@x{\@s{97.38} \.{\land} ( m2 . type\@s{1.1} \.{=}\@w{2b} ) \.{\implies}
 MsgInv2b ( m2 ) ) \.{'} \@s{4.0} {\BY} {\DEF} MsgInv}%
\begin{lcom}{18.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 Proves \ensuremath{MsgInv1b} using two cases. \@pfstepnum{7}{1} is for \ensuremath{m2 \in msgs}. \@pfstepnum{7}{2} is for the increment \ensuremath{m2 \in msgs' \setminus msgs}. 
\end{cpar}\end{lcom}
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  ( m2 . type \.{=}\@w{1b} \.{\implies}
 MsgInv1b ( m2 ) ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.} {\CASE} m2\@s{0.83} \.{\in} msgs\@s{2.0}
 {\BY}\@pfstepnum{7}{1} ,\,\@pfstepnum{5}{13} ,\,\@pfstepnum{5}{1} ,\,
 Phase1bVotedForInv ,\,\@pfstepnum{4}{2}\  {\DEF} MsgInv ,\, MsgInv1b ,\,}%
\@x{\@s{36.44} TypeOK ,\, Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{2.} {\CASE} m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  m2 \.{=} m1\@s{2.0} {\BY}\@pfstepnum{5}{1}
 ,\,\@pfstepnum{7}{2} ,\,\@pfstepnum{5}{13}\  {\DEF} Send}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{7}{2}
 ,\,\@pfstepnum{5}{13} ,\, Phase1bVotedForInv ,\,\@pfstepnum{4}{2}
 ,\,\@pfstepnum{5}{2} ,\,\@pfstepnum{5}{4} ,\,\@pfstepnum{5}{12}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{2}{1} ,\,}%
 \@x{\@s{36.89}\@pfstepnum{8}{1}\  {\DEF} Send ,\, TypeOK ,\, MsgInv ,\,
 Messages ,\, MsgInv1b}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}
 ,\,\@pfstepnum{7}{2}\ }%
\begin{lcom}{18.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
Proves \ensuremath{MsgInv2a} and \ensuremath{MsgInv2b} using invariance lemma for \ensuremath{Phase1b} because it does not send \textsf{2a} or \textsf{2b} messages.
\end{cpar}\end{lcom}
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  ( ( m2 . type \.{=}\@w{2a} \.{\implies}
 MsgInv2a ( m2 ) ) \.{\land} ( m2 . type \.{=}\@w{2b} \.{\implies} MsgInv2b (
 m2 ) ) ) \.{'}}%
 \@x{\@s{35.1} {\BY}\@pfstepnum{5}{13} ,\, Phase1bVotedForInv
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{4}{2} ,\,\@pfstepnum{3}{1} ,\,
 SafeAtStable ,\,\@pfstepnum{2}{1}\  {\DEF} Send ,\, TypeOK ,\,}%
\@x{\@s{35.1} MsgInv ,\, Messages ,\, MsgInv2a ,\, MsgInv2b}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\ }%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{14} is the simple case of preemption and uses the invariance lemmas for \ensuremath{Phase1b} and \ensuremath{SafeAt}.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{14.} {\CASE} {\lnot} ( m . bal \.{>} aBal [ a ] )\,
 {\BY}\@pfstepnum{5}{14} ,\, Phase1bVotedForInv ,\,\@pfstepnum{4}{2}
 ,\,\@pfstepnum{5}{2} ,\,\@pfstepnum{5}{4} ,\,\@pfstepnum{5}{12}
 ,\,\@pfstepnum{5}{1} ,\,}%
 \@x{\@s{32.44} SafeAtStable ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{2}{1}\ 
 {\DEF} Send ,\, TypeOK ,\, MsgInv ,\, Messages ,\, MsgInv1b ,\, MsgInv2a ,\,
 MsgInv2b}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{13}
 ,\,\@pfstepnum{5}{14}\ }%
\begin{lcom}{10.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{4}{3} proves \ensuremath{MsgInv'} for \ensuremath{Phase2a}. Each of \@pfstepnum{5}{4-6} proves a conjunct of \ensuremath{MsgInv}.
\end{cpar}\end{lcom}
 \@x{\@s{8.0}\@pfstepnum{4}{3.}\  {\ASSUME} {\NEW} p \.{\in} {\mathcal{P}} ,\,
 Phase2a ( p )\@s{2.0} {\PROVE} MsgInv \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\SUFFICES} {\ASSUME} {\NEW} m \.{\in} msgs
 \.{'}}%
 \@x{\@s{60.31} {\PROVE} ( \.{\land} ( m . type \.{=}\@w{1b}
 \.{\implies} MsgInv1b ( m )) \.{\land} ( m . type\@s{1.1} \.{=}\@w{2a} \@s{0.29}
 \.{\implies} MsgInv2a ( m ))}%
 \@x{\@s{93.38} \.{\land} ( m . type\@s{1.1} \.{=}\@w{2b} \.{\implies}
 MsgInv2b ( m )) ) \.{'} \@s{4.0} {\BY} {\DEF} MsgInv}%
\@x{\@s{12.0}\@pfstepnum{5}{}\  {\DEFINE} b \.{\defeq} pBal [ p ]}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} Q \.{\in} {\mathcal{Q}} ,\, S \.{\in}
 {\SUBSET} \{ m2 \.{\in} msgs \.{:} ( m2 . type \.{=}\@w{1b} ) \.{\land} ( m2
 . bal \.{=} b ) \} \.{:}}%
 \@x{\@s{35.1} \.{\land} \A\, a \.{\in} Q \.{:} \E\, m2 \.{\in} S \.{:} m2 .
 from \.{=} a}%
 \@x{\@s{35.1} \.{\land} Send ( [ type \.{\mapsto}\@w{2a} ,\, bal \.{\mapsto}
 b ,\, from \.{\mapsto} p ,\, propSV \.{\mapsto} PropSV ( {\UNION}
 \{ m2 . voted \.{:} m2 \.{\in} S \} ) ] )}%
\@x{\@s{31.1} {\BY}\@pfstepnum{4}{3}\  {\DEF} Phase2a}%
 \@x{\@s{12.0}\@pfstepnum{5}{2.}\  b \.{=} pBal \.{'} [ p ] \.{\land} b
 \.{\in} {\mathcal{B}}\@s{2.0} {\BY}\@pfstepnum{4}{3}\  {\DEF} Phase2a ,\, TypeOK}%
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} m2 . type \.{=}\@w{2a} \.{\land} m2 . bal
 \.{=} b\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{4} proves \ensuremath{MsgInv1b'}. % for \ensuremath{Phase2a}. 
 It uses invariance lemma for \ensuremath{Phase2a}, because \ensuremath{Phase2a} does not send 1b messages.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  ( m . type \.{=}\@w{1b} \.{\implies}
 MsgInv1b ( m ) ) \.{'}}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} ( m . type \.{=}\@w{1b}
 ) \.{'}\@s{2.0} {\PROVE} MsgInv1b ( m ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  ( m . bal \.{\leq} aBal [ m . from ] )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{4}{3} ,\,\@pfstepnum{5}{3}
 ,\,\@pfstepnum{3}{1} ,\, Phase2aVotedForInv {\DEF} TypeOK ,\, Messages ,\,}%
\@x{\@s{35.1} MsgInv ,\, Phase2a ,\, MsgInv1b}%
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  ( \A\, r \.{\in} m . voted \.{:} VotedForIn
 ( m . from ,\, r . bal ,\, r . slot ,\, r . val ) ) \.{'}\@s{2.0}
 {\BY}\@pfstepnum{4}{3} ,\,\@pfstepnum{5}{3} ,\,\@pfstepnum{3}{1} ,\,}%
 \@x{\@s{35.1} Phase2aVotedForInv {\DEF} TypeOK ,\, Messages ,\, MsgInv ,\,
 MsgInv1b}%
 \@x{\@s{16.0}\@pfstepnum{6}{3.}\  \A\, s \.{\in} {\mathcal{S}} \.{:} MaxBalInSlot
 ( m . voted ,\, s ) \.{=} MaxBalInSlot ( m . voted ,\, s ) \.{'}\@s{2.0}
 {\BY} {\DEF} MaxBalInSlot}%
 \@x{\@s{16.0}\@pfstepnum{6}{4.}\  ( \A\, b2 \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b2 \.{\in} MaxBalInSlot ( m . voted ,\,
 s ) \.{+} 1 \.{\dotdot} m . bal \.{-} 1 \.{\implies}}%
\@x{\@s{40.22} {\lnot} VotedForIn ( m . from ,\, b2 ,\, s ,\, v ) ) \.{'}}%
 \@x{\@s{35.1} {\BY}\@pfstepnum{4}{3} ,\,\@pfstepnum{5}{3}
 ,\,\@pfstepnum{3}{1} ,\, Phase2aVotedForInv ,\,\@pfstepnum{6}{3}\  {\DEF}
 TypeOK ,\, Messages ,\, MsgInv ,\, MsgInv1b}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2} ,\,\@pfstepnum{6}{4}\  {\DEF} MsgInv1b}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{5} proves \ensuremath{MsgInv2a'}. Each of \@pfstepnum{6}{2-4} proves a conjunct of \ensuremath{MsgInv2a} using the increment approach. The increment is \ensuremath{m2} in \@pfstepnum{8}{2} of \@pfstepnum{7}{9}.
%annie: not clear which is an increment case. sc-all of them are. Should I mention the exact step number in the comments for each case?
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{5.}\  ( m . type \.{=}\@w{2a} \.{\implies}
 MsgInv2a ( m ) ) \.{'}}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} ( m . type \.{=}\@w{2a}
 ) \.{'}\@s{2.0} {\PROVE} MsgInv2a ( m ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\DEFINE} VS \.{\defeq} {\UNION} \{ m2 .
 voted \.{:} m2 \.{\in} S \}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  \A\, a \.{\in} Q \.{:} aBal [ a ] \.{\geq}
 b\@s{2.0} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{2} ,\,\@pfstepnum{3}{1}\ 
 {\DEF} MsgInv ,\, TypeOK ,\, Messages ,\, MsgInv1b}%
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  ( \A\, d \.{\in} m . propSV \.{:} SafeAt (
 m . bal ,\, d . slot ,\, d . val ) ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  \A\, d \.{\in} [ slot \.{:} UnusedS ( VS
 ) ,\, val \.{:} {\mathcal{V}} ] \.{\,\backslash\,} {\emptyset} \.{:} SafeAt ( b ,\, d .
 slot ,\, d . val )}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\SUFFICES} {\ASSUME} {\NEW} d \.{\in} [ slot
 \.{:} UnusedS ( VS ) ,\, val \.{:} {\mathcal{V}} ] \.{\,\backslash\,} {\emptyset}
 \@s{2.0} {\PROVE} SafeAt ( b ,\, d . slot ,\, d . val )}%
\@x{\@s{36.89} {\OBVIOUS}}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  \A\, m2 \.{\in} S \.{:} {\nexists}\, d2
 \.{\in} m2 . voted \.{:} d . slot \.{=} d2 . slot\@s{2.0} {\BY} {\DEF}
 UnusedS}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  \A\, m2 \.{\in} S \.{:} MaxBalInSlot (
 m2 . voted ,\, d . slot ) \.{+} 1 \.{=} 0\@s{2.0} {\BY}\@pfstepnum{8}{1}\ 
 {\DEF} MaxBalInSlot}%
 \@x{\@s{24.0}\@pfstepnum{8}{3.}\  \A\, m2 \.{\in} S ,\, b2 \.{\in} {\mathcal{B}}
 ,\, s \.{\in} {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b2 \.{\in} MaxBalInSlot (
 m2 . voted ,\, s ) \.{+} 1 \.{\dotdot} m2 . bal \.{-} 1 \.{\implies}}%
 \@x{\@s{47.1} {\lnot} VotedForIn ( m2 . from ,\, b2 ,\, s ,\, v )\@s{2.0}
 {\BY} {\DEF} MsgInv ,\, MsgInv1b}%
 \@x{\@s{24.0}\@pfstepnum{8}{4.}\  \A\, v \.{\in} {\mathcal{V}} ,\, b2 \.{\in}
 {\mathcal{B}} ,\, a \.{\in} Q \.{:} b2 \.{\in} 0 \.{\dotdot} b \.{-} 1
 \.{\implies} {\lnot} VotedForIn ( a ,\, b2 ,\, d . slot ,\, v )}%
 \@x{\@s{43.1} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{8}{2}
 ,\,\@pfstepnum{8}{3}\  {\DEF} UnusedS ,\, TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{4}
 ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{6}{1}\  {\DEF} SafeAt ,\, NewSV
 ,\, UnusedS ,\, WontVoteIn ,\, TypeOK ,\, Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{2.}\  \A\, d \.{\in} [ slot \.{:} UnusedS ( VS
 ) ,\, val \.{:} {\mathcal{V}} ] \.{\,\backslash\,} {\emptyset} \.{:} SafeAt ( b ,\, d .
 slot ,\, d . val ) \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{1} ,\, SafeAtStable
 ,\,}%
 \@x{\@s{39.1}\@pfstepnum{3}{1} ,\,\@pfstepnum{2}{1} ,\,\@pfstepnum{5}{2}\ 
 {\DEF} NewSV ,\, UnusedS ,\, TypeOK ,\, Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{3.}\  \A\, d \.{\in} NewSV ( VS ) \.{:}
 SafeAt ( b ,\, d . slot ,\, d . val ) \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{2}
 ,\, Misc {\DEF} NewSV}%
 \@x{\@s{20.0}\@pfstepnum{7}{4.}\  \A\, d \.{\in} MaxBSV ( VS ) \.{:}
 SafeAt ( b ,\, d . slot ,\, d . val )}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\SUFFICES} {\ASSUME} {\NEW} d \.{\in}
 MaxBSV ( VS ) ,\, {\NEW} b2 \.{\in} {\mathcal{B}} ,\, b2 \.{\in} 0
 \.{\dotdot} ( b \.{-} 1 )}%
 \@x{\@s{72.31} {\PROVE} \E\, Q2 \.{\in} {\mathcal{Q}} \.{:} \A\, a \.{\in}
 Q2 \.{:} \.{\lor} VotedForIn ( a ,\, b2 ,\, d . slot ,\, d . val )}%
 \@x{\@s{180.63}  \.{\lor} WontVoteIn ( a ,\, b2 ,\, d . slot ) \@s{4.0} {\BY} {\DEF} SafeAt}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\DEFINE} max \.{\defeq} MaxBalInSlot ( VS
 ,\, d . slot )}%
\@x{\@s{24.0}\@pfstepnum{8}{}\  {\USE} {\DEF} MaxBSV}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  max \.{\in} {\mathcal{B}}\@s{2.0} {\BY} MaxBinSType
 ,\, MaxBinSNoSlot {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  \A\, m2 \.{\in} S \.{:} MaxBalInSlot (
 m2 . voted ,\, d . slot ) \.{\leq} max}%
 \@x{\@s{43.1} {\BY} \A\, m2 \.{\in} S \.{:} m2 . voted \.{\subseteq} VS ,\,
 MaxBinSSubsets {\DEF} MaxBSV ,\, TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{3.}\  {\nexists}\, d2 \.{\in} VS \.{:} ( d2 . bal
 \.{>} d . bal \.{\land} d2 . slot \.{=} d . slot )}%
 \@x{\@s{43.1} {\BY} \A\, d2 \.{\in} VS \.{:} {\lnot} ( {\lnot} ( d2 . bal
 \.{\leq} d . bal ) \.{\land} d2 . slot \.{=} d . slot ) {\DEF} MaxBSV
 ,\, TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{4.}\  VS \.{\subseteq} [ bal \.{:} {\mathcal{B}}
 ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]\@s{2.0} {\BY}\@pfstepnum{3}{1}\ 
 {\DEF} TypeOK ,\, Messages}%
\@x{\@s{24.0}\@pfstepnum{8}{5.}\  max \.{=} d . bal}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\SUFFICES} {\ASSUME} max \.{\neq} d .
 bal\@s{2.0} {\PROVE} {\FALSE} \@s{4.0} {\OBVIOUS}}%
\@x{\@s{28.0}\@pfstepnum{9}{1.} {\CASE} max \.{>} d . bal}%
\@x{\@s{32.0}\@pfstepnum{10}{}\  {\HIDE} {\DEF} VS}%
 \@x{\@s{32.0}\@pfstepnum{10}{1.}\  \E\, d2 \.{\in} VS \.{:} d2 . bal \.{=}
 max \.{\land} d2 . slot \.{=} d . slot\@s{2.0} {\BY}\@pfstepnum{8}{4}
 ,\,\@pfstepnum{8}{1} ,\, MaxBinSExists}%
 \@x{\@s{32.0}\@pfstepnum{10}{}\  {\QED} {\BY}\@pfstepnum{10}{1}
 ,\,\@pfstepnum{8}{3} ,\,\@pfstepnum{9}{1}\ }%
 \@x{\@s{28.0}\@pfstepnum{9}{2.} {\CASE} max \.{<} d . bal\@s{2.0} {\BY}
 MaxBinSNoMore ,\,\@pfstepnum{9}{2}\  {\DEF} MaxBSV ,\, TypeOK ,\,
 Messages}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{9}{1}
 ,\,\@pfstepnum{9}{2} ,\,\@pfstepnum{8}{1}\  {\DEF} {\mathcal{B}} ,\, TypeOK ,\,
 Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{6.} {\CASE} b2 \.{\in} max \.{+} 1 \.{\dotdot} b
 \.{-} 1}%
\@x{\@s{28.0}\@pfstepnum{9}{}\  {\HIDE} {\DEF} max}%
 \@x{\@s{28.0}\@pfstepnum{9}{1.}\  \A\, m2 \.{\in} S ,\, b3 \.{\in} {\mathcal{B}}
 ,\, v \.{\in} {\mathcal{V}} \.{:} b3 \.{\in} MaxBalInSlot ( m2 . voted ,\, d .
 slot ) \.{+} 1 \.{\dotdot} b \.{-} 1 \.{\implies}}%
\@x{\@s{51.1} {\lnot} VotedForIn ( m2 . from ,\, b3 ,\, d . slot ,\, v )}%
\@x{\@s{47.1} {\BY} {\DEF} MsgInv ,\, TypeOK ,\, Messages ,\, MsgInv1b}%
 \@x{\@s{28.0}\@pfstepnum{9}{2.}\  \A\, m2 \.{\in} S ,\, v \.{\in} {\mathcal{V}}
 \.{:} {\lnot} VotedForIn ( m2 . from ,\, b2 ,\, d . slot ,\, v )}%
 \@x{\@s{47.1} {\BY}\@pfstepnum{8}{6} ,\,\@pfstepnum{9}{1}
 ,\,\@pfstepnum{8}{2} ,\,\@pfstepnum{8}{1} ,\, MaxBinSType {\DEF} TypeOK ,\,
 Messages ,\, Send}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{5}{1}
 ,\,\@pfstepnum{8}{6} ,\,\@pfstepnum{6}{1} ,\,\@pfstepnum{9}{2}\  {\DEF}
 MsgInv ,\, MsgInv1b ,\, TypeOK ,\, Messages ,\, WontVoteIn ,\,}%
\@x{\@s{40.89} MaxBSV}%
\@x{\@s{24.0}\@pfstepnum{8}{7.} {\CASE} b2 \.{=} max}%
 \@x{\@s{32.0}\@pfstepnum{9}{1.}\  \E\, a \.{\in} {\mathcal{A}} ,\, m2 \.{\in} S
 \.{:} m2 . from \.{=} a \.{\land} \E\, d2 \.{\in} m2 . voted \.{:}}%
 \@x{\@s{55.1} d2 . bal \.{=} d . bal \.{\land} d2 . slot \.{=} d . slot
 \.{\land} d2 . val \.{=} d . val}%
\@x{\@s{51.1} {\BY} {\DEF} MaxBalInSlot ,\, TypeOK ,\, Messages}%
 \@x{\@s{32.0}\@pfstepnum{9}{2.}\  \E\, a \.{\in} {\mathcal{A}} \.{:} VotedForIn (
 a ,\, b2 ,\, d . slot ,\, d . val )}%
 \@x{\@s{51.1} {\BY}\@pfstepnum{8}{7} ,\,\@pfstepnum{9}{1}
 ,\,\@pfstepnum{8}{5}\  {\DEF} MsgInv ,\, TypeOK ,\, Messages ,\, MsgInv1b}%
 \@x{\@s{32.0}\@pfstepnum{9}{3.}\  \A\, q \.{\in} Q ,\, v2 \.{\in} {\mathcal{V}}
 \.{:} VotedForIn ( q ,\, b2 ,\, d . slot ,\, v2 ) \.{\implies} v2 \.{=} d .
 val}%
 \@x{\@s{51.1} {\BY}\@pfstepnum{9}{2} ,\, VotedOnce ,\, QuorumAssumption
 {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{32.0}\@pfstepnum{9}{4.}\  \A\, q \.{\in} Q \.{:} aBal [ q ] \.{>}
 b2\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF} MsgInv ,\, TypeOK ,\, Messages
 ,\, MsgInv1b}%
 \@x{\@s{32.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{8}{7}
 ,\,\@pfstepnum{9}{3} ,\,\@pfstepnum{9}{4}\  {\DEF} WontVoteIn}%
\@x{\@s{24.0}\@pfstepnum{8}{8.} {\CASE} b2 \.{\in} 0 \.{\dotdot} max \.{-} 1}%
 \@x{\@s{32.0}\@pfstepnum{9}{1.}\  \E\, a \.{\in} {\mathcal{A}} \.{:} VotedForIn (
 a ,\, d . bal ,\, d . slot ,\, d . val )}%
 \@x{\@s{51.1} {\BY}\@pfstepnum{8}{8} ,\,\@pfstepnum{8}{2}\  {\DEF} MsgInv
 ,\, TypeOK ,\, Messages ,\, MsgInv1b}%
 \@x{\@s{32.0}\@pfstepnum{9}{2.}\  SafeAt ( d . bal ,\, d . slot ,\, d . val
 )\@s{2.0} {\BY}\@pfstepnum{9}{1} ,\, VotedInv {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{32.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{8}{8}
 ,\,\@pfstepnum{9}{2} ,\,\@pfstepnum{8}{5}\  {\DEF} SafeAt ,\, MsgInv ,\,
 TypeOK ,\, Messages ,\, MaxBalInSlot}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{6}
 ,\,\@pfstepnum{8}{7} ,\,\@pfstepnum{8}{8} ,\,\@pfstepnum{8}{1}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{5.}\  MaxBSV ( VS ) \.{\subseteq} [ bal
 \.{:} {\mathcal{B}} ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]\@s{2.0} {\BY}
 {\DEF} MaxBSV ,\, TypeOK ,\, Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{6.}\  \A\, d \.{\in} MaxBSV ( VS ) \.{:}
 SafeAt ( b ,\, d . slot ,\, d . val ) \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{4}
 ,\, SafeAtStable ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{7}{5}
 ,\,\@pfstepnum{2}{1} ,\,\@pfstepnum{5}{2}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{7.}\  \A\, d \.{\in} MaxSV ( VS ) \.{:} SafeAt ( b
 ,\, d . slot ,\, d . val ) \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{6}
 ,\,\@pfstepnum{7}{5}\  {\DEF} MaxSV}%
 \@x{\@s{20.0}\@pfstepnum{7}{8.}\  \A\, d \.{\in} MaxSV ( VS ) \.{\cup}
 NewSV ( VS ) \.{:} SafeAt ( b ,\, d . slot ,\, d . val )
 \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{7} ,\,\@pfstepnum{7}{3}\ }%
 \@x{\@s{20.0}\@pfstepnum{7}{9.}\  ( \A\, m2 \.{\in} msgs \.{:} m2 . type
 \.{=}\@w{2a} \.{\implies} \A\, d \.{\in} m2 . propSV \.{:} SafeAt ( m2 .
 bal ,\, d . slot ,\, d . val ) ) \.{'}}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\SUFFICES} {\ASSUME} {\NEW} m2 \.{\in} msgs
 \.{'} ,\, ( m2 . type \.{=}\@w{2a} ) \.{'} ,\, {\NEW} d \.{\in} m2 .
 propSV}%
 \@x{\@s{72.31} {\PROVE} ( SafeAt ( m2 . bal ,\, d . slot ,\, d . val
 ) ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.} {\CASE} m2 \.{\in} msgs\@s{2.0}
 {\BY}\@pfstepnum{3}{1} ,\, SafeAtStable ,\,\@pfstepnum{8}{1}
 ,\,\@pfstepnum{2}{1}\  {\DEF} MsgInv ,\, MsgInv2a ,\, Messages ,\, TypeOK}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.} {\CASE} m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs}%
 \@x{\@s{28.0}\@pfstepnum{9}{1.}\  SafeAt ( m2 . bal ,\, d . slot ,\, d . val
 ) \.{'}\@s{2.0} {\BY}\@pfstepnum{7}{8} ,\,\@pfstepnum{8}{2}
 ,\,\@pfstepnum{5}{1} ,\,\@pfstepnum{5}{2}\  {\DEF} Send ,\, PropSV}%
 \@x{\@s{28.0}\@pfstepnum{9}{}\  {\QED} {\BY}\@pfstepnum{3}{1}
 ,\,\@pfstepnum{9}{1}\  {\DEF} Send ,\, TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{1}
 ,\,\@pfstepnum{8}{2}\ }%
\@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{9}\ }%
\begin{lcom}{18.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
The increment is \ensuremath{m2} in \@pfstepnum{7}{1}.
\end{cpar}\end{lcom}
 \@x{\@s{16.0}\@pfstepnum{6}{3.}\  ( \A\, d1 ,\, d2 \.{\in} m . propSV \.{:}
 d1 . slot \.{=} d2 . slot \.{\implies} d1 \.{=} d2 ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} \A\, d1 ,\, d2 \.{\in} m2 . propSV\@s{0.84}
 \.{:} d1 . slot \.{=} d2 . slot \.{\implies} d1 \.{=} d2}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  VS \.{\in} {\SUBSET} [ bal \.{:} {\mathcal{B}}
 ,\, slot \.{:} {\mathcal{S}} ,\, val \.{:} {\mathcal{V}} ]\@s{2.0} {\BY} {\DEF} Messages
 ,\, TypeOK}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  \A\, r1 ,\, r2 \.{\in} MaxBSV ( VS )
 \.{:} r1 . slot \.{=} r2 . slot \.{\implies} r1 . bal \.{=} r2 . bal\@s{2.0}
 {\BY}\@pfstepnum{8}{1}\  {\DEF} MaxBSV}%
 \@x{\@s{24.0}\@pfstepnum{8}{3.}\  MaxBSV ( VS ) \.{\subseteq} VS\@s{2.0}
 {\BY}\@pfstepnum{8}{1}\  {\DEF} MaxBSV}%
 \@x{\@s{24.0}\@pfstepnum{8}{4.}\  \A\, r1 ,\, r2 \.{\in} MaxBSV ( VS )
 \.{:} r1 . bal \.{=} r2 . bal \.{\land} r1 . slot \.{=} r2 . slot
 \.{\implies} r1 . val \.{=} r2 . val}%
\@x{\@s{43.1} {\BY}\@pfstepnum{8}{3} ,\, VotedUnion}%
 \@x{\@s{24.0}\@pfstepnum{8}{5.}\  \A\, r1 ,\, r2 \.{\in} MaxBSV ( VS )
 \.{:} r1 . slot \.{=} r2 . slot \.{\implies} r1 . bal \.{=} r2 . bal
 \.{\land} r1 . val \.{=} r2 . val}%
 \@x{\@s{43.1} {\BY}\@pfstepnum{8}{4} ,\,\@pfstepnum{8}{2}
 ,\,\@pfstepnum{8}{3} ,\,\@pfstepnum{8}{1}\ }%
 \@x{\@s{24.0}\@pfstepnum{8}{6.}\  \A\, r1 ,\, r2 \.{\in} MaxSV ( VS ) \.{:} r1
 . slot \.{=} r2 . slot \.{\implies} r1 \.{=} r2\@s{2.0}
 {\BY}\@pfstepnum{8}{5}\  {\DEF} MaxSV}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{8}{6} ,\, Misc
 ,\,\@pfstepnum{5}{1}\  {\DEF} PropSV ,\, Send}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}\  {\DEF} MsgInv
 ,\, MsgInv2a}%
\begin{lcom}{18.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
The increment is \ensuremath{m1,m2} in \@pfstepnum{7}{2}.
\end{cpar}\end{lcom}
 \@x{\@s{16.0}\@pfstepnum{6}{4.}\  ( \A\, m2 \.{\in} msgs \.{:} ( m2 . type
 \.{=}\@w{2a} \.{\land} m2 . bal \.{=} m . bal ) \.{\implies} ( m2 \.{=} m )
 ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  \A\, m2 \.{\in} msgs \.{:} ( m2 . type
 \.{=}\@w{2a} ) \.{\implies} ( m2 . bal \.{\neq} b )\@s{2.0}
 {\BY}\@pfstepnum{4}{3}\  {\DEF} Phase2a}%
 \@x{\@s{20.0}\@pfstepnum{7}{2.}\  \A\, m1 ,\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} m1 \.{=} m2\@s{2.0} {\BY}\@pfstepnum{4}{3}\ 
 {\DEF} Phase2a ,\, Send}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{1}
 ,\,\@pfstepnum{7}{2} ,\,\@pfstepnum{5}{3} ,\,\@pfstepnum{2}{1}
 ,\,\@pfstepnum{3}{1}\  {\DEF} MsgInv ,\, MsgInv2a}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{2}
 ,\,\@pfstepnum{6}{3} ,\,\@pfstepnum{6}{4}\  {\DEF} MsgInv2a}%
\iffalse
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{6} proves \ensuremath{MsgInv2b'}. Since \ensuremath{Phase2a} sends \ensuremath{2a} messages, the proof is simple.  %annie: the reason does say anything really. 
\end{cpar}\end{lcom}
\fi
 \@x{\@s{12.0}\@pfstepnum{5}{6.}\  ( ( m . type \.{=}\@w{2b} ) \.{\implies}
 MsgInv2b ( m ) ) \.{'}\@s{2.0} {\BY}\@pfstepnum{5}{3} ,\,\@pfstepnum{5}{1}
 ,\, m . type \.{=}\@w{2b} \.{\implies} m \.{\in} msgs ,\,}%
 \@x{\@s{31.1}\@pfstepnum{3}{1} ,\,\@pfstepnum{4}{3}\  {\DEF} TypeOK ,\,
 Messages ,\, MsgInv ,\, Phase2a ,\, Send ,\, MsgInv2b}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{4}
 ,\,\@pfstepnum{5}{5} ,\,\@pfstepnum{5}{6}\ }%
\begin{lcom}{10.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{4}{4} proves \ensuremath{MsgInv'} for \ensuremath{Phase2b}. Each of \@pfstepnum{5}{2-4} proves a conjunct of \ensuremath{MsgInv}.
\end{cpar}\end{lcom}
 \@x{\@s{8.0}\@pfstepnum{4}{4.}\  {\ASSUME} {\NEW} a \.{\in} {\mathcal{A}} ,\,
 Phase2b ( a )\@s{2.0} {\PROVE} MsgInv \.{'}}%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\SUFFICES} {\ASSUME} {\NEW} m \.{\in} msgs
 \.{'}}%
 \@x{\@s{60.31} {\PROVE} ( \.{\land} ( m . type \.{=}\@w{1b} )
 \.{\implies} MsgInv1b ( m ) \.{\land} ( m . type\@s{1.1} \.{=}\@w{2a} )\@s{0.29}
 \.{\implies} MsgInv2a ( m )}%
 \@x{\@s{93.38} \.{\land} ( m . type\@s{1.1} \.{=}\@w{2b} ) \.{\implies}
 MsgInv2b ( m ) ) \.{'} \@s{4.0} {\BY} {\DEF} MsgInv}%
 \@x{\@s{12.0}\@pfstepnum{5}{1.}\  {\PICK} m1 \.{\in} msgs \.{:} Phase2b ( a )
 {\bang} ( m1 )\@s{2.0} {\BY}\@pfstepnum{4}{4}\  {\DEF} Phase2b}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{2} proves \ensuremath{MsgInv1b'} for\ensuremath{Phase2b}. Invariance lemmas do not apply because the 3rd conjunct in \ensuremath{MsgInv1b} quantifies over \ensuremath{2b} messages negatively 
 %annie: does it matter to be negative
 %sc: if it was not negative, the invariance lemma would have worked. 
 %annie: i remember this one now.  thanks!
 ---\ensuremath{VotedForIn(a, b, s, v)} means acceptor \ensuremath{a} has sent a \textsf{2b} message voting \ensuremath{\langle b, s, v\rangle}.
 %\ensuremath{Phase2bVotedForInv} fails to work here for \@pfstepnum{6}{2}.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{2.}\  ( ( m . type \.{=}\@w{1b} ) \.{\implies}
 MsgInv1b ( m ) ) \.{'}}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\SUFFICES} {\ASSUME} ( m . type \.{=}\@w{1b}
 ) \.{'}\@s{2.0} {\PROVE} MsgInv1b ( m ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.}\  ( m . bal \.{\leq} aBal [ m . from ]
 \.{\land} \A\, r \.{\in} m . voted \.{:} VotedForIn ( m . from ,\, r . bal
 ,\, r . slot ,\, r . val ) ) \.{'}}%
 \@x{\@s{35.1} {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{1}
 ,\,\@pfstepnum{4}{4} ,\, Phase2bVotedForInv {\DEF} MsgInv ,\, MsgInv1b ,\,
 TypeOK ,\,}%
\@x{\@s{35.1} Messages ,\, Send}%
 \@x{\@s{16.0}\@pfstepnum{6}{2.}\  ( \A\, b \.{\in} {\mathcal{B}} ,\, s \.{\in}
 {\mathcal{S}} ,\, v \.{\in} {\mathcal{V}} \.{:} b \.{\in} MaxBalInSlot ( m . voted ,\, s
 ) \.{+} 1 \.{\dotdot} m . bal \.{-} 1 \.{\implies}}%
\@x{\@s{40.22} {\lnot} VotedForIn ( m . from ,\, b ,\, s ,\, v ) ) \.{'}}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\SUFFICES} {\ASSUME} {\NEW} b \.{\in}
 {\mathcal{B}} \.{'} ,\, {\NEW} s \.{\in} {\mathcal{S}} \.{'} ,\, {\NEW} v \.{\in} {\mathcal{V}}
 \.{'} ,\,}%
 \@x{\@s{98.91} ( b \.{\in} MaxBalInSlot ( m . voted ,\, s ) \.{+} 1
 \.{\dotdot} m . bal \.{-} 1 ) \.{'}}%
 \@x{\@s{68.31} {\PROVE} ( {\lnot} VotedForIn ( m . from ,\, b ,\, s
 ,\, v ) ) \.{'} \@s{4.0} {\OBVIOUS}}%
 \@x{\@s{20.0}\@pfstepnum{7}{1.}\  {\lnot} VotedForIn ( m . from ,\, b ,\, s
 ,\, v )\@s{2.0} {\BY}\@pfstepnum{5}{1}\  {\DEF} Send ,\, MsgInv ,\, TypeOK
 ,\, Messages ,\, MsgInv1b}%
 \@x{\@s{20.0}\@pfstepnum{7}{2.} {\CASE} m . from \.{\neq} a \.{\lor} {\lnot}
 ( m1 . bal \.{\geq} aBal [ a ] )\@s{2.0} {\BY}\@pfstepnum{5}{1}
 ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{7}{2} ,\,\@pfstepnum{7}{1}\  {\DEF}
 VotedForIn ,\,}%
\@x{\@s{38.44} TypeOK ,\, Messages ,\, Send}%
 \@x{\@s{20.0}\@pfstepnum{7}{3.} {\CASE} m . from \.{=} a \.{\land} ( m1 . bal
 \.{\geq} aBal [ a ] )}%
 \@x{\@s{24.0}\@pfstepnum{8}{1.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} m2 . bal \.{=} m1 . bal\@s{2.0}
 {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{7}{3} ,\,\@pfstepnum{6}{1}
 ,\,\@pfstepnum{7}{3}\  {\DEF} Send ,\, TypeOK}%
 \@x{\@s{24.0}\@pfstepnum{8}{2.}\  \A\, m2 \.{\in} msgs \.{'}
 \.{\,\backslash\,} msgs \.{:} m2 . bal \.{\neq} b\@s{2.0}
 {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{7}{3} ,\,\@pfstepnum{6}{1}
 ,\,\@pfstepnum{7}{3} ,\,\@pfstepnum{8}{1}\  {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{24.0}\@pfstepnum{8}{}\  {\QED} {\BY}\@pfstepnum{7}{3}
 ,\,\@pfstepnum{7}{1} ,\,\@pfstepnum{8}{2}\  {\DEF} VotedForIn ,\, TypeOK ,\,
 Messages}%
 \@x{\@s{20.0}\@pfstepnum{7}{}\  {\QED} {\BY}\@pfstepnum{7}{2}
 ,\,\@pfstepnum{7}{3}\  {\DEF} TypeOK ,\, Messages}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\  {\DEF} MsgInv1b}%
\iffalse
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{3} proves \ensuremath{MsgInv2a'}. Because \ensuremath{Phase2b} sends \ensuremath{2b} messages, it uses invariance lemma for \ensuremath{SafeAt}.  %annie: the reason seems to be say anything.
\end{cpar}\end{lcom}
\fi
 \@x{\@s{12.0}\@pfstepnum{5}{3.}\  ( ( m . type \.{=}\@w{2a} ) \.{\implies}
 MsgInv2a ( m ) ) \.{'}\@s{2.0} {\BY} SafeAtStable ,\,\@pfstepnum{3}{1}
 ,\,\@pfstepnum{4}{4} ,\,\@pfstepnum{2}{1}\  {\DEF} MsgInv ,\, MsgInv2a ,\,}%
\@x{\@s{31.1} TypeOK ,\, Messages ,\, Phase2b ,\, Send}%
\begin{lcom}{14.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{5}{4} proves \ensuremath{MsgInv2b'}. It uses two cases: the second case, \@pfstepnum{6}{2}, is for the increment \ensuremath{m}.
\end{cpar}\end{lcom}
 \@x{\@s{12.0}\@pfstepnum{5}{4.}\  ( ( m . type \.{=}\@w{2b} ) \.{\implies}
 MsgInv2b ( m ) ) \.{'}}%
 \@x{\@s{16.0}\@pfstepnum{6}{1.} {\CASE} {\lnot} ( m1 . bal \.{\geq} aBal [ a
 ] ) \.{\lor} m \.{\in} msgs\@s{2.0} {\BY}\@pfstepnum{5}{1}
 ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{6}{1}\  {\DEF} TypeOK ,\, Messages ,\,}%
\@x{\@s{34.44} Send ,\, MsgInv ,\, MsgInv2b}%
 \@x{\@s{16.0}\@pfstepnum{6}{2.} {\CASE} m1 . bal \.{\geq} aBal [ a ]
 \.{\land} m \.{\in} msgs \.{'} \.{\,\backslash\,} msgs\@s{2.0}
 {\BY}\@pfstepnum{5}{1} ,\,\@pfstepnum{3}{1} ,\,\@pfstepnum{6}{2}\  {\DEF}
 TypeOK ,\, Send ,\, MsgInv2b}%
 \@x{\@s{16.0}\@pfstepnum{6}{}\  {\QED} {\BY}\@pfstepnum{6}{1}
 ,\,\@pfstepnum{6}{2}\ }%
 \@x{\@s{12.0}\@pfstepnum{5}{}\  {\QED} {\BY}\@pfstepnum{5}{2}
 ,\,\@pfstepnum{5}{3} ,\,\@pfstepnum{5}{4}\  {\DEF} MsgInv2b}%
\begin{lcom}{10.5}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
 \@pfstepnum{4}{5} proves \ensuremath{MsgInv'} for \ensuremath{Preempt}.  It uses the invariance lemma for \ensuremath{Preempt}, since \ensuremath{Preempt} does not send messages.
\end{cpar}\end{lcom}
 \@x{\@s{8.0}\@pfstepnum{4}{5.} {\CASE} \E\, p \.{\in} {\mathcal{P}} \.{:}
 Preempt ( p )\@s{2.0} {\BY}\@pfstepnum{4}{5} ,\, PreemptVotedForInv
 ,\,\@pfstepnum{3}{1} ,\, SafeAtStable ,\,}%
 \@x{\@s{26.44}\@pfstepnum{2}{1}\  {\DEF} Preempt ,\, MsgInv ,\, TypeOK ,\,
 Messages ,\, MsgInv1b ,\, MsgInv2a ,\, MsgInv2b}%
 \@x{\@s{8.0}\@pfstepnum{4}{}\  {\QED} {\BY}\@pfstepnum{4}{1}
 ,\,\@pfstepnum{4}{2} ,\,\@pfstepnum{4}{3} ,\,\@pfstepnum{4}{4}
 ,\,\@pfstepnum{4}{5} ,\,\@pfstepnum{2}{1}\  {\DEF} Next}%
 \@x{\@s{4.0}\@pfstepnum{3}{}\  {\QED} {\BY}\@pfstepnum{3}{1}
 ,\,\@pfstepnum{3}{2} ,\,\@pfstepnum{3}{3}\  {\DEF} Inv ,\, vars ,\, Next}%
 \@x{\@s{4.0}\@pfstepnum{2}{2.} {\CASE} {\UNCHANGED} vars\@s{2.0}
 {\BY}\@pfstepnum{2}{2}\  {\DEF} vars ,\, Inv ,\, TypeOK ,\, AccInv ,\,
 MsgInv ,\, VotedForIn ,\,}%
 \@x{\@s{22.44} SafeAt ,\, WontVoteIn ,\, MaxBalInSlot ,\, MsgInv1b ,\,
 MsgInv2a ,\, MsgInv2b}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{2}{2}\ }%
 \@x{\@pfstepnum{1}{}\  {\QED} {\BY}\@pfstepnum{1}{1} ,\,\@pfstepnum{1}{2} ,\,
 \texttt{PTL} {\DEF} Spec}%
\@pvspace{8.0pt}%
\begin{lcom}{0}%
\begin{cpar}{0}{F}{F}{0}{0}{}%
\ensuremath{Safety} asserts that \ensuremath{Spec} implies that \ensuremath{Safe} always holds.%It uses (1) theorem \ensuremath{Invariant} which states that \ensuremath{Spec} implies all the invariants in \ensuremath{Inv} always hold and (2) \ensuremath{Inv \Rightarrow Safe}.
\end{cpar}%
\end{lcom}%
\@x{ {\THEOREM} Safety \.{\defeq} Spec \.{\implies} {\Box} Safe}%
\@x{\@pfstepnum{1}{}\  {\USE} {\DEF} {\mathcal{B}}}%
\@x{\@pfstepnum{1}{1.}\  Inv \.{\implies} Safe}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\SUFFICES} {\ASSUME} Inv ,\, {\NEW} v1
 \.{\in} {\mathcal{V}} ,\,\@s{2.0} {\NEW} v2 \.{\in} {\mathcal{V}} ,\, {\NEW} s \.{\in}
 {\mathcal{S}} ,\, {\NEW} b1 \.{\in} {\mathcal{B}} ,\, {\NEW} b2 \.{\in} {\mathcal{B}} ,\,}%
 \@x{\@s{82.91} ChosenIn ( b1 ,\, s ,\, v1 ) ,\, ChosenIn ( b2 ,\, s ,\, v2 )
 ,\, b1 \.{\leq} b2}%
\@x{\@s{52.31} {\PROVE} v1 \.{=} v2 \@s{4.0} {\BY} {\DEF} Safe ,\, Chosen}%
\@x{\@s{4.0}\@pfstepnum{2}{1.} {\CASE} b1 \.{=} b2}%
 \@x{\@s{8.0}\@pfstepnum{3}{1.}\  \E\, a \.{\in} {\mathcal{A}} \.{:} VotedForIn (
 a ,\, b1 ,\, s ,\, v1 ) \.{\land} VotedForIn ( a ,\, b1 ,\, s ,\, v2 )}%
\@x{\@s{27.1} {\BY}\@pfstepnum{2}{1} ,\, QuorumAssumption {\DEF} ChosenIn}%
 \@x{\@s{8.0}\@pfstepnum{3}{}\  {\QED} {\BY}\@pfstepnum{3}{1} ,\, VotedOnce
 {\DEF} Inv}%
\@x{\@s{4.0}\@pfstepnum{2}{2.} {\CASE} b1 \.{<} b2}%
 \@x{\@s{8.0}\@pfstepnum{3}{1.}\  SafeAt ( b2 ,\, s ,\, v2 )\@s{2.0} {\BY}
 VotedInv ,\, QuorumAssumption {\DEF} ChosenIn ,\, Inv}%
 \@x{\@s{8.0}\@pfstepnum{3}{2.}\  {\PICK} Q1 \.{\in} {\mathcal{Q}} \.{:} \A\, a
 \.{\in} Q1 \.{:} VotedForIn ( a ,\, b1 ,\, s ,\, v1 )\@s{2.0} {\BY} {\DEF}
 ChosenIn}%
 \@x{\@s{8.0}\@pfstepnum{3}{3.}\  {\PICK} Q2 \.{\in} {\mathcal{Q}} \.{:} \A\, a
 \.{\in} Q2 \.{:} VotedForIn ( a ,\, b1 ,\, s ,\, v2 ) \.{\lor} WontVoteIn (
 a ,\, b1 ,\, s )\@s{2.0} {\BY}\@pfstepnum{3}{1} ,\,\@pfstepnum{2}{2}\ 
 {\DEF} SafeAt}%
 \@x{\@s{8.0}\@pfstepnum{3}{}\  {\QED} {\BY}\@pfstepnum{3}{2}
 ,\,\@pfstepnum{3}{3} ,\, QuorumAssumption ,\, VotedOnce {\DEF} WontVoteIn
 ,\, Inv}%
 \@x{\@s{4.0}\@pfstepnum{2}{}\  {\QED} {\BY}\@pfstepnum{2}{1}
 ,\,\@pfstepnum{2}{2}\ }%
\@x{\@pfstepnum{1}{}\  {\QED} {\BY} Invariant ,\,\@pfstepnum{1}{1} ,\, \texttt{PTL}}%
\@x{}\bottombar\@xx{}%

